Reference Frame in General Relativity

A reference frame in event space is a smooth field of orthonormal bases. Every reference frame is equipped by anholonomic coordinates. Using anholonomic coordinates allows to find out relative speed of two observers and appropriate Lorentz transformation. Synchronization of a reference frame is an anholonomic time coordinate. Simple calculations show how synchronization influences time measurement in the vicinity of the Earth. Measurement of Doppler shift from the star orbiting the black hole helps to determine mass of the black hole. According observations of Sgr A, if non orbiting observer estimates age of S2 about 10 Myr, this star is 0.297 Myr younger.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{texSpaceTime}{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84 (1966)
}%

\BiblioItem{texGenRelativity}{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{texGenRelativity}{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{texAffine,texGeomObject}{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{texAffine}{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric-affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{texAffine}{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{texAffine}{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\BiblioItem{texAffine}{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%

\BiblioItem{texTidal,texAffine,texGeomObject}{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{texTidal,texNewton}{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{texNewton}{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{texNewton}{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric-affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{texLagrange}{Weinberg}
{
Steven Weinberg. The Quantum Theory of Fields. Cambridge university press.
}%

\BiblioItem{texLagrange}{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{texLagrange}{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{texTidal}{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{texTidal}{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{texTidal}{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{texReferenceFrame,texFiberedAlgebra}{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{texFiberedAlgebra,texTstarMorphism}{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{texGeomObject}{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{texAffine,texRepresentation,texBasis,texDrcBasis,texVectorSpace,texLinearMap}
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem{texDrcBasis,texBasis}{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{texGenRelativity}{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{texGenRelativity}{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{texGenRelativity}{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{texGenRelativity}{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{texGenRelativity}{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity}{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{texGenRelativity,texTidal}{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{texBiring,texVectorSpace}{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{texBiring,texVectorSpace}
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{texVectorSpace}{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{texVectorSpace}{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{texVectorSpace}{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{texVectorSpace}{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{texVectorSpace}{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{texDrcReferenceFrame,texRefernceFrame,texGeomObject,texLie,texLieRepresentation}{0412.391}
{
Александр Клейн,
Многообразие базисов,
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2004)
}%

\BiblioItem{texAffine}{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2004)
}%

\BiblioItem{texTidal}{0405.028}
{
Aleks Kleyn, Metric-Affine Manifold,
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2004)
}%

\BiblioItem{texFiberedAlgebra,texBundleRelation,texTstarMorphism}{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2007)
}%

\BiblioItem{texBundleRelation,texPrefaceRelation}{0702.561}
{
Александр Клейн,
Расслоенная алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

%\BiblioItem{texBasis,texLinearMap}{math.RA-0501237}
%{
%Александр Клейн,
%Векторное пространство над телом,\\
%eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2005)
%}%

\BiblioItem{texPolymodule}{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Skew-Field, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\ifx\texBiring\Defined
\else
\BiblioItem{texVectorSpace,texFiberedAlgebra}{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2006)
}%
\fi

\ifx\texBundleRelation\Defined
\else
\BiblioItem{texFiberedMorphism}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\ifx\PrintBook\Defined
\BiblioItem{texPrefaceRelation}{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%
\fi

\BiblioItem{texHomotopy}{q-alg-9705009}
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{texSpaceTime}{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81 (1967)
}%

\BiblioItem{texPrefaceRelation}{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem{texBundleRelation,texPrefaceRelation,texTstarMorphism,texBundle}
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem{texBundle}
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{texFiberedAlgebra}{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{texBundleRelation}{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{texBundle,texCartesian,texFiberedAlgebra,texBundleRelation,texFiberedMorphism}
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{texCalculus}{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{texCalculus}{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{texCalculus}{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem{texFiberedMorphism}{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{texFiberedAlgebra,texFiberedMorphism}{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{texFiberedMorphism}{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{texFiberedMorphism}{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\CloseBiblio



==> Gen.Relativity.Russian.tex <==
%auto-ignore
\def\texGenRelativity{}
\ifx\PrintBook\Defined
				\chapter{Приложения в общей теории относительности}
\fi

			\section{Синхронизация системы отсчёта}
			\label{section: Synchronization of Reference Frame}

Так как наблюдатель пользуется ортогональным базисом для измерения в каждой точке,
мы можем ожидать, что он также пользуется неголономными координатами.
Мы так же видим, что координата времени вдоль локальной системы отсчёта
является собственным временем наблюдателя.
Так как система отсчёта состоит из локальных систем отсчёта,
мы ожидаем, что их собственные времена
синхронизированы.

Мы определяем \AddIndex{синхронизацию системы отсчёта}{synchronization of reference frame}
как неголономную координату времени.

Так как синхронизация - это неголономная координата, это порождает
новые физические явления,
которые мы должны иметь в виду, когда работаем с сильными гравитационными полями
или выполняем
точные измерения. Ниже я опишу одно из этих явлений.

			\section{Неголономные координаты в гравитационном поле центрального тела}
			\label{section: Anholonomic Coordinates in Central Body Gravitational Field}

Мы будем изучать наблюдателя, вращающегося вокруг центрального тела.
Результаты оценочны и хороши, когда эксцентриситет около $0$,
так как мы будем изучать круговую орбиту.
Тем не менее, основная цель этой оценки - показать, что мы имеем
измеримое действие неголономности.

Мы пользуемся метрикой Шварцшильда для центрального тела
	\begin{equation}
ds^2 = \frac{r-r_g} r c^2 dt^2
- \frac r {r-r_g} dr^2 - r^2 d\phi^2 - r^2 sin^2 \phi d\theta^2
	\label{eq: Schwarzschild}
	\end{equation}
$$r_g = \frac {2 G m} {c^2}$$
$G$ - гравитационная константа, $m$ - масса центрального тела,
$c$ - скорость света.

Эта метрика имеет связность
\[\Gamma^0_{10}=\frac {r_g} {2r(r-r_g)}\]
\[\Gamma^1_{00}=\frac {r_g(r-r_g)} {2r^3}\]
\[\Gamma^1_{11}=-\frac {r_g} {2r(r-r_g)}\]
\[\Gamma^1_{22}=-(r-r_g)\]
\[\Gamma^1_{33}=-(r-r_g)\sin^2\phi\]
\[\Gamma^2_{12}=-\frac 1 r\]
\[\Gamma^2_{33}=-\sin\phi\cos\phi\]
\[\Gamma^3_{13}=-\frac 1 r\]
\[\Gamma^3_{23}=\cot\phi\]

%Curvature tensor is
%\section{Эффект Допплера}

Я хочу показать ещё один способ
рассчёта эффекта Допплера. Эффект Допплера в гравитационном поле является
хорошо изученным явлением, однако метод, который я покажу полезен, чтобы
лучше понять физику гравитационного поля.

Мы можем описать движение фотона в гравитационном поле,
пользуясь его волновым вектором $k^i$. Длина этого вектора равна 0;
$\frac {k^i} {dx^i} = const$; траектория является
геодезической, и следовательно, координаты этого вектора удовлетворяют
дифференциальному уравнению
	\begin{equation}
dk^i = -\Gamma^i_{kl}k^k dx^l
	\label{eq: Transport}
	\end{equation}

Мы ищем частоту $\omega$ света
и $k^0$ пропорционально $\omega$.
Рассмотрим радиальное движение фотона. В этом случае волновой вектор имеет вид 
$k=(k^0,k^1,0,0)$.
В центральном поле с метрикой
\eqref{eq: Schwarzschild} мы можем выбрать
\[k^0=\frac \omega c \sqrt{\frac r {r-r_g}}\]
\[k^1=\omega \sqrt{\frac {r-r_g} r}\]
\[dt=\frac {k^0} {k^1} dr= \frac 1 c \frac r {r-r_g}dr\]
Тогла уравнение \eqref{eq: Transport} принимает вил
\[dk^0=-\Gamma^0_{10}(k^1 dt + k^0 dr)\]
\[d\left(\frac\omega c \sqrt{\frac r {r-r_g}}\right)=
-\frac{r_g \omega} {2r(r-r_g)}\left(\sqrt{\frac {r-r_g} r}\frac r {r-r_g}
+\sqrt{\frac r {r-r_g}}\right)\frac {dr} c\]
\[d\omega \sqrt{\frac r {r-r_g}}-\omega\frac 1 2 \sqrt{\frac {r-r_g}r}
\frac {r_gdr} {(r-r_g)^2}
=-\frac {r_g\omega dr} {r(r-r_g)}\sqrt{\frac r {r-r_g}}\]
\[\frac  {d\omega} \omega
=-\frac {r_g} {2r(r-r_g)}dr\]
\[\ln  \omega
=\frac 1 2 \ln \frac r {r-r_g} + \ln C\]
Если мы определим $\omega = \omega_0$, когда $r=\infty$, мы получим окончательно 
\[\omega
=\omega_0\sqrt{\frac r {r-r_g}}\]

			\section{Задержка времени в гравитационном поле центрального тела}
			\label{section: Time Delay in Central Body Gravitational Field}

Мы изучим вращение вокруг центрального тела.
Результаты являются только оценкой и хороши, когда эксцентриситет около $0$,
так как мы изучаем круговые орбиты.
Основная задача этой оценки - показать, что мы имеем измеримый эффект негологомности.

Давайте сравним измерения двух наблюдателей. Первый наблюдатель
зафиксировал своё положение в гравитационном поле
$$t=\frac s  c \sqrt{\frac r {r-r_g}}$$ $$r=const, \phi=const, \theta=const$$
Второй наблюдатель вращается вокруг центра поля с постоянной скоростью
$$t=s \sqrt{\frac r {(r-r_g) c^2 - \alpha^2 r^3}}$$
$$\phi=\alpha\ s \sqrt{\frac r {(r-r_g) c^2 - \alpha^2 r^3}}$$
$$r=const,\theta=const$$
Мы выберем натуральный параметр для обоих наблюдателей.

Второй наблюдатель начинает своё путешествие,
когда $s=0$, и завершает его, когда возвращается к той же точке пространства.
Так как $\phi$ - циклическая координата, второй наблюдатель завершает своё путешествие,
когда $\phi=2\pi$. В этой точке мы имеем
$$s_2=\frac{2\pi} \alpha \sqrt{\frac{(r-r_g) c^2 - \alpha^2 r^3} r}$$
$$t=T=\frac{2\pi} \alpha$$
Значение натурального параметра первого наблюдателя в этой точке
$$s_1=\frac{2\pi} \alpha c\sqrt{\frac{r-r_g} r}$$
Разница между их собственными временами
$$
\Delta s = s_1 - s_2
=\frac{2\pi} \alpha
\left(c\sqrt{\frac{r-r_g} r}-\sqrt{\frac{(r-r_g) c^2 - \alpha^2 r^3} r}\right)
$$
Мы определили разницу в сантиметрах. Чтобы получить разницу в секундах,
мы должны делить обе части на c.
$$\Delta t = \frac{2\pi} \alpha
\left(\sqrt{\frac{r-r_g} r}-\sqrt{\frac{r-r_g} r - \frac{\alpha^2 r^2} {c^2}}\right)$$

Перейдём к конкретным данным.

Масса Солнца равна $1.989_{10}33$ г, Земля вращается вокруг Солнца на
расстоянии $1.495985_{10}13$ см от его центра напротяжение $365.257$ дней.
В этом случае мы получим
$\Delta t = 0.155750625445089$ сек. Меркурий вращается вокруг Солнца на
расстоянии $5.791_{10}12$ см от его центра напротяжение $58.6462$ дней.
В этом случае мы получим
$\Delta t = 0.145358734930827$ сек.

Масса Земли равна $5.977_{10}27$ г. Космический корабль,
который вращается вокруг Земли на
расстоянии $6.916_{10}8$ см от его центра напротяжение $95.6$ мин
имеет $\Delta t = 1.8318_{10}-6$ сек.
Луна вращается вокруг Земли на
расстоянии $3.84_{10}10$ см от его центра напротяжение $27.32$ дней.
В этом случае мы получим
$\Delta t = 1.372_{10}-5$ сек.

Для лучшего представления я поместил эти данные в
таблицы \ref{table: Effect of Anholonomic Coordinates, Sun},
\ref{table: Effect of Anholonomic Coordinates, Earth},
и \ref{table: Effect of Anholonomic Coordinates, Sgr A}.

Так как часы первого наблюдателя в момент встречи показывают большее
значение, он оценивает возраст второго наблюдателя
старше реального. Так, если взять параметры орбиты S2 из \citeBib{Ghez},
то мы получим, что за 10 Myr S2 будет моложе на .297 Myr по сравнению
с оценкой неподвижного наблюдателя.

\begin{table}[h]
\caption{Солнце - центральное тело, масса - $1.989_{10}33$ г}
\label{table: Effect of Anholonomic Coordinates, Sun}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
спутник&Земля&Меркурий\\
\hline
расстояние, см&$1.495985_{10}13$&$5.791_{10}12$\\
\hline
период вращения, дней&$365.257$&$58.6462$\\
\hline
задержка времени, сек&$0.15575$&$0.14536$\\
\hline
\end{tabular}
\]
\end{table}

\begin{table}[h]
\caption{Земля - центральное тело, масса - $5.977_{10}27$ г}
\label{table: Effect of Anholonomic Coordinates, Earth}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
спутник&космический корабль&Луна\\
\hline
расстояние, см&$6.916_{10}8$&$3.84_{10}10$\\
\hline
период вращения&$95.6$ mins&$27.32$ дней\\
\hline
задержка времени, сек&$1.8318_{10}-6$&$1.372_{10}-5$\\
\hline
\end{tabular}
\]
\end{table}

\begin{table}[h]
\caption{Sgr A - центральное тело, S2 - спутник}
\label{table: Effect of Anholonomic Coordinates, Sgr A}
\noindent\[
\begin{tabular}{|c|c|c|}
\hline
масса, $M_\odot$&$4.1_{10}6$&$3.7_{10}6$\\
\hline
расстояние, см&$1.4692_{10}16$&$1.1565_{10}16$\\
\hline
период вращения, лет&$15.2$&$15.2$\\
\hline
задержка времени, мин&$164.7295$&$153.8326$\\
\hline
\end{tabular}
\]
\end{table}

\section{Преобразование Лоренца в орбитальном направлении}
			\label{section: Lorentz Transformation in Orbital Direction}

Причина задержки времени, которую мы оценили выше, находится в преобразовании Лоренца
между стационарным и вращающимся наблюдателями.
Это значит, что мы имеем вращение в плоскости $(e_{(0)}, e_{(2)})$.
Базисные вектора для стационарного наблюдателя - это
\[e_{(0)}=(\frac 1 c \sqrt{\frac r {r-a}}, 0, 0, 0)\]
\[e_{(2)}=(0, 0, \frac 1 r, 0)\]
Мы предположим, что для вращающегося наблюдателя изменение $\phi$ и $t$
пропорциональны и
\[d\phi=\omega dt\]
Единичный вектор скорости в этом случае должен быть пропорционален вектору
	\begin{equation}
(1, 0, \omega, 0)
	\label{NewVectorE2}
	\end{equation}
Длина этого вектора
	\begin{equation}
L^2=\frac {r-a} r c^2 - r^2 \omega^2
	\label{LengthNewVectorE2}
	\end{equation}
Мы видим в этом выражении очень знакомый узор и ожидаем, что линейная
скорость вращающегося наблюдателя $V = \omega r$.

Тем не менее, мы должны помнить, что мы выполняем измерение в гравитационном
поле и координаты являются лишь ярлыками для разметки точек в пространстве времени.
Это значит, что нам нужен корректный метод для измерения скорости.

Если объект движется от точки $(t, \phi)$ к точке $(t+dt, \phi+d\phi)$
мы должны измерить пространственные и временные интервалы между этими точками.
Мы предположим, что в обеих точках имеются наблюдатели $A$ и $B$.
Наблюдатель $A$ посылает одновременно световой сигнал $B$ и мяч, который имеет
угловую скорость $\omega$. Каждый раз, когда
наблюдатель $B$ получает какую-то информацию, он посылает световой сигнал
обратно $A$.

Когда $A$ получает первый сигнал, он может оценить расстояние до $B$.
Когда $A$ получает второй сигнал, он может оценить, как долго двигался мяч до $B$.

Время путешествия света в обоих направлениях одно и тоже.
Траектория света определена уравнением $ds^2=0$.
В данном случае мы имеем
\[\frac {r-r_g} r c^2 dt^2 - r^2 d\phi^2 = 0\]
Когда свет возвращается к наблюдателю $A$, изменение $t$ равно
\[dt=2 \sqrt{\frac r {r-r_g}} c^{-1}r d\phi\]
Собственное время первого наблюдателя равно
\[ds^2= \frac {r-r_g} r c^2 4 \frac r {r-r_g}c^{-2}r^2 d\phi^2\]
Следовательно, пространственное расстояние
\[L=r d\phi\]
Когда объект, движущийся с угловой скорость $\omega$, прибывает в $B$,
изменение $t$ равно $\frac {d\phi} \omega$.
Собственное время в этой точке равно 
\[ds^2 = \frac {r - r_g} r c^2 d\phi^2 \omega^{-2}\]
\[T = \sqrt{\frac {r - r_g} r} \omega^{-1} d\phi\]
Следовательно, наблюдатель $A$ измеряет скорость
\[V=\frac L T = \sqrt{\frac r {r - r_g}} r\omega\]

Мы можем использовать скорость $V$ как параметр преобразования Лоренца.
Тогда длина
\eqref{LengthNewVectorE2} вектора \eqref{NewVectorE2} равна
\[L=\sqrt{\frac {r-r_g} r \left(c^2 - \frac r {r-r_g}r^2 \omega^2\right)}=
\sqrt{\frac {r-r_g} r} c\sqrt{\left(1 - \frac {V^2}{c^2}\right)}\]
Следовательно, временной орт движущегося наблюдателя
\[e'_{(0)}=\left(\frac 1 L, 0, \frac \omega L, 0\right)\]
\[e'_{(0)}=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,
\omega \sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0\right)\]
Пространственный орт $e'_{(2)}=(A,0,B,0)$ ортогонален $e'_{(0)}$ и имеет длину $-1$. Следовательно,
	\begin{equation}
\frac {r-r_g} r c^2\frac 1 L A - r^2 \frac \omega L B = 0
	\label{NewVectorE0_1}
	\end{equation}
	\begin{equation}
\frac {r-r_g} r c^2 A^2 - r^2 B^2 = -1
	\label{NewVectorE0_2}
	\end{equation}
Мы можем выразить $A$ из \eqref{NewVectorE0_1}
\[A = c^{-2}\frac r{r-r_g} r^2 \omega B\]
и подставить в \eqref{NewVectorE0_2}
\[ c^{-2}\frac r{r-r_g} r^4 \omega^2 B^2 - r^2 B^2 = -1\]
\[\frac {V^2}{c^2} r^2 B^2 - r^2 B^2 = -1\]
Окончательно пространственный орт в направлении движения
\[e'_{(2)}=\left(c^{-2}\frac r{r-r_g} r \omega \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},
0,\frac 1 r \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},0\right)\]
\[e'_{(2)}=\left(c^{-2}\sqrt{\frac r{r-r_g}} \frac V {\sqrt{1 - \frac {V^2}{c^2}}},
0,\frac 1 r \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}},0\right)\]

Следовательно, мы получим преобразование
	\begin{equation}
	\begin{split}
{e'}_{(0)}=\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac V  c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(2)}
\\
{e'}_{(2)}=\frac V c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(2)}
	\end{split}
	\label{Lorentz}
	\end{equation}
Если стационарный наблюдатель посылает свет в радиальном направлении,
вращающийся наблюдатель наблюдает эффект Допплера
$$
\omega'=\frac \omega {\sqrt{1 - \frac {V^2} {c^2}}}
$$
Мы должны добавить эффект Допплера для гравитационного поля,
если движущийся наблюдатель получает радиальную волну, которая пришла из
бесконечности. В этом случае эффект Допплера примет форму
$$
\omega'=\sqrt{\frac r {r-r_g}}\frac \omega {\sqrt{ 1 - \frac {V^2} {c^2}}}
$$

Мы приводим оценку для динамики звезды S2, которая вращается вокруг Sgr A
в таблицах \ref{table:DShift1S2} и \ref{table:DShift2S2}.
Таблицы основаны на двух различных оценках для массы Sgr A.

\begin{sloppypar}
Если мы возьмём массу Sgr $4.1_{10}6 M_\odot$ \citeBib{Ghez}, то
в перицентре (расстояние $1.868_{10}15$ см) S2 имеет скорость $738767495.4$ см/сек
и эффект Допплера равен $\omega'/\omega=1.000628$. В этом случае мы измеряем длину $2.16474 \mu m$
для волны, излучаемой с длиной $2.1661 \mu m$ (Br $\gamma$).
В апоцентре (расстояние $2.769_{10}16cm$) S2 имеет скорость $49839993.28cm/s$
и эффект Допплера равен $\omega'/\omega=1.0000232$. Мы измеряем длину $2.166049 \mu m$
для той же самой волны.
Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$13.098\AA$.
\end{otherlanguage}

Если мы возьмём массу Sgr $3.7_{10}6 M_\odot$ \citeBib{Schodel}, то
в перицентре (расстояние $1.805_{10}15cm$) S2 имеет скорость $713915922.3cm/s$
и эффект Допплера равен $\omega'/\omega=1.000587$. В этом случае мы измеряем длину $2.16483 \mu m$
для волны, излучаемой с длиной $2.1661 \mu m$ (Br $\gamma$).
В апоцентре (расстояние $2.676_{10}16cm$) S2 имеет скорость $48163414.05cm/s$
и эффект Допплера равен $\omega'/\omega=1.00002171$. Мы измеряем длину $2.1666052 \mu m$
для той же самой волны.
Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$12.232\AA$.
\end{otherlanguage}
\end{sloppypar}

\begin{table}[h]
\caption{эффект Допплера на Земле для волны, излучаемой с S2;
масса Sgr A равна $4.1_{10}6 M_\odot$ \citeBib{Ghez}}
\label{table:DShift1S2}
\begin{tabular}{|c|c|c|}
\hline
&перицентр&апоцентр\\
\hline
расстояние см&$1.868_{10}15$&$2.769_{10}16$\\
\hline
скорость см/s&$738767495.4$&$49839993.28$\\
\hline
$\omega'/\omega$&$1.000628$&$1.0000232$\\
\hline
излучаемая волна $(Br\ \gamma)\ \mu m$& $2.1661$&$2.1661$\\
\hline
наблюдаемая волна $\mu m$&$2.16474$ &$2.166049$\\
\hline
\end{tabular}

Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$13.098\AA$
\end{otherlanguage}
\end{table}

\begin{table}[h]
\caption{эффект Допплера на Земле для волны, излучаемой с S2;
масса Sgr A равна $3.7_{10}6 M_\odot$ \citeBib{Schodel}}
\label{table:DShift2S2}
\begin{tabular}{|c|c|c|}
\hline
&перицентр&апоцентр\\
\hline
расстояние см&$1.805_{10}15$&$2.676_{10}16$\\
\hline
скорость см/s&$713915922.3$&$48163414.05$\\
\hline
$\omega'/\omega$&$1.000587$&$1.00002171$\\
\hline
излучаемая волна $(Br\ \gamma)\ \mu m$& $2.1661$&$2.1661$\\
\hline
наблюдаемая волна $\mu m$&$2.16483$ &$2.1666052$\\
\hline
\end{tabular}

Разность между двумя измерениями длины волны равна
\begin{otherlanguage}{english}
$12.232\AA$
\end{otherlanguage}
\end{table}

Разность между двумя измерениями длины волны в перицентре равна
\begin{otherlanguage}{english}
$0.9\AA$.
\end{otherlanguage}
Анализируя эти данные, мы приходим к заключению, что
использование эффекта Допплера может помочь улучшить оценку
массы Sgr A.

\section{Преобразование Лоренца в радиальном направлении}

Мы видим, что преобразование Лоренца в орбитальном направлении имеет знакомый вид.
Очень интересно увидеть, какой вид это преобразование имеет в радиальном направлении.
Мы начнём с процедуры измерения скорости и будем пользоваться координатной скоростью $v$
	\begin{equation}
dr=vdt
	\label{eq: RadialSpeed}
	\end{equation}
Время путешествия света в обоих направлениях одно и тоже.
Траектория света определена уравнением $ds^2=0$.
\[\frac {r-r_g} r c^2 dt^2 - \frac r {r-r_g} dr^2 = 0\]
Когда свет возвращается к наблюдателю $A$, изменение $t$ равно
\[dt=2 \frac r {r-r_g} c^{-1} dr\]
Собственное время наблюдателя $A$ равно
	\begin{align*}
ds^2&= \frac {r-r_g} r c^2 4 \frac {r^2} {{r-r_g}^2}c^{-2}dr^2=\\
&=  4 \frac r {r-r_g}dr^2
	\end{align*}
Следовательно, пространственное расстояние равно
\[L=\sqrt{\frac r {r-r_g}} dr\]
Когда объект, движущийся со скоростью \eqref{eq: RadialSpeed}, прибывает в $B$
изменение $t$ равно $\frac {dr} v$.
Собственное время наблюдателя $A$ в этой точке 
\[ds^2 = \frac {r - r_g} r c^2 dr^2 v^{-2}\]
\[T = \sqrt{\frac {r - r_g} r} v^{-1} dr\]
Следовательно, наблюдатель $A$ измеряет скорость
	\begin{align*}
V&=\frac L T =
=\frac{\sqrt{\frac r {r-r_g}} dr}{\sqrt{\frac {r - r_g} r} v^{-1} dr}=\\
&=\frac r {r-r_g} v
	\end{align*}

Теперь мы готовы найти преобразование Лоренца.
Базисные вектора для стационарного наблюдателя - это
\[e_{(0)}=\left(\frac 1 c \sqrt{\frac r {r-r_g}}, 0, 0, 0\right)\]
\[e_{(1)}=\left(0,  \sqrt{\frac {r-r_g} r},0, 0\right)\]

Единичный вектор скорости должен быть пропорционален вектору
	\begin{equation}
(1, v, 0, 0)
	\label{eq: NewRadialVectorE1}
	\end{equation}
Длина этого вектора
	\begin{equation}
	\begin{split}
L^2&=\frac {r-r_g} r c^2 - \frac r {r-r_g} v^2=\\
&=\frac {r-r_g} r c^2\left(1 - \frac {V^2}{c^2}\right)
	\label{eq: LengthNewRadialVectorE1}
	\end{split}
	\end{equation}
Следовательно, временной орт движущегося наблюдателя
	\begin{align*}
e'_{(0)}&=\left(\frac 1 L,  \frac v L,0, 0\right)=\\
&=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 
v \sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,0\right)\\
&=\left(\sqrt{\frac r {r-r_g}} c^{-1}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 
\frac V c \sqrt{\frac {r-r_g} r}\frac 1 {\sqrt{\left(1 - \frac {V^2}{c^2}\right)}}, 0,0\right)
	\end{align*}
Пространственный орт $e'_{(1)}=(A,B,0,0)$ ортогонален $e'_{(0)}$ и имеет длину $-1$. Следовательно,
	\begin{equation}
\frac {r-r_g} r c^2\frac 1 L A - \frac r {r-r_g} \frac v L B = 0
	\label{NewRadialVectorE0_1}
	\end{equation}
	\begin{equation}
\frac {r-r_g} r c^2 A^2 - \frac r {r-r_g} B^2 = -1
	\label{NewRadialVectorE0_2}
	\end{equation}
Мы можем выразить $A$ из \eqref{NewRadialVectorE0_1}
\[A = c^{-2}\frac {r^2}{(r-r_g)^2} v B = c^{-2}\frac r{r-r_g} V B\]
и подставить в \eqref{NewRadialVectorE0_2}
\[\frac {r-r_g} r c^2 c^{-4}\frac {r^2}{(r-r_g)^2} V^2 B^2 - \frac r {r-r_g} B^2 = -1\]
\[\frac r{r-r_g} B^2\left(1- \frac{V^2}{c^2} \right) = 1\]
\[ B^2 = \frac{r-r_g} r\frac 1{1- \frac{V^2}{c^2} }\]
\[ B = \sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }\]
	\begin{align*}
A &= c^{-2}\frac r{r-r_g} V \sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }\\
&= c^{-2} V \sqrt{\frac r{r-r_g}}\frac 1{\sqrt{1- \frac{V^2}{c^2}} }
	\end{align*}
Окончательно пространственный орт в направлении движения
\[e'_{(1)}=\left(c^{-2} V \sqrt{\frac r{r-r_g}}\frac 1{\sqrt{1- \frac{V^2}{c^2}} },
\sqrt{\frac{r-r_g} r}\frac 1{\sqrt{1- \frac{V^2}{c^2}} },0,0\right)\]

Следовательно, мы подучаем преобразование в знакомой форме
	\begin{equation}
	\begin{split}
{e'}_{(0)}=\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac V  c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(1)}
\\
{e'}_{(1)}=\frac V c \frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(0)} +
\frac 1 {\sqrt{1 - \frac {V^2}{c^2}}} e_{(1)}
	\end{split}
	\label{RadialLorentz}
	\end{equation}

			\section{Эффект Допплера в пространстве Фридмана}

Мы рассмотрим другой пример в пространстве Фридмана. Метрика
пространства имеет вид
$$ds^2 = a^2 (dt^2
- d\chi^2 - \sin^2\chi (d\theta^2 - \sin^2 \theta d\phi^2))
$$
для закрытой модели и
$$ds^2 = a^2 (dt^2
- d\chi^2 - \sinh^2\chi (d\theta^2 - \sin^2 \theta d\phi^2))
$$
для открытой модели. Связность пространства
($\alpha$, $\beta$ принимают значения 1, 2, 3)
\[\Gamma^0_{00}=\frac {\dot{a}} a\]
\[\Gamma^0_{\alpha\alpha}=-\frac {\dot{a}} {a^2}g_{\alpha\alpha}\]
\[\Gamma^\alpha_{0\beta}=\frac {\dot{a}} a\delta^\alpha_\beta\]

Поскольку пространства однородно, для нас не имеет значение
направление распространения света.
В этом случае
\[dk^0=-\Gamma^0_{ij}k^i k^j\]
Так как $k$ - изотропный вектор, касательный к его траектории, мы имеем
\[dx^\alpha=\frac {k^\alpha} {k^0}dt\]
Так как $k^0=\frac \omega a$, то
\[d\frac \omega a=-\frac {da} {a^2}\omega+\frac {da} {\omega a}g_{\alpha\alpha}k^\alpha k^\alpha=
-2\frac {da} {a^2}\omega\]
\[ad\omega+\omega da=0\]
\[a\omega=const\]
Следовательно, когда $a$ растёт,
$\omega$ становится меньше и длина волны растёт. 

$a$ растёт, когда свет путешествует сквозь пространство время,
и это приводит к красному смещению.
Причиной наблюдаемого красного смещения
является не разбегание галактик,
а изменение геометрии.

Рассмотрим теперь как красное смещение меняется во времени,
если начальная и конечная точки не движутся.
Для простоты я буду изменять только $\chi$. $\chi_1$ - начальное значение
и $\chi_2$ - конечное значение. Так как на траектории
света $dt=d\chi$, мы имеем
\[\chi = \chi_1 + t - t_1\ \ \ \ t_2 = \chi_2 - \chi_1 + t_1\]
Следовательно $a(t_1) \omega_1 = a(t_2) \omega_2$.
Смещение Допплера имеет вид
\[K(t_1) =\frac {\omega_2} {\omega_1} = \frac {a(t_1)} {a(t_2)}\]
Если начальное время изменяется t'1 = t1 + dt, то K(t1 + dt) = a(t1 + dt) / a(t2 + dt) 
Производная $K$ по времени имеет вид    
\[\dot{K} = \frac {\dot{a}_1 a_2 - a_1 \dot{a}_2} {a_2^2}\]

Для замкнутого пространства $a = \cosh t$. Тогда $\dot{a} = \sinh t$. 
\[\dot{K} = \frac{\sinh t_1 \cosh t_2 - \sinh t_2 \cosh t_1} {\cosh^2 t_2}
= \frac{\sinh(t_1 - t_2)} {\cosh^2 t_2}\] 
$K$ уменьшается, когда $t_1$ увеличивается. 

			\section{Преобразование Лоренца в пространстве Фридмана}

Чтобы изучить преобразование Лоренца в пространстве Фридмана,
я хочу воспользоваться метрикой в форме
\[ds^2=c^2 dt^2 -a^2(d\chi^2 + b^2(d\theta^2 - \sin^2 \theta d\phi^2))\]
У меня есть два наблюдателя. Один не движется и имеет скорость $(1,0,0,0)$,
а другой движется вдоль $\chi$ и его скорость
имеет вид $C=(1,v,0,0)$, и мы положим $V=a v$.

Метрика диагональна и координаты $\theta, \phi$ не меняются.
У нас возникает преобразование в плоскости $t, \chi$.

Единичная скорость первого наблюдателя имеет вид
\[e_0 = (\frac 1 c , 0, 0, 0)\]
и вектор, ортогональный ей, имеет вид
\[e_1 = (0, \frac 1 a , 0, 0)\]

Длина вектора $C$ имеет вид
\[L=\sqrt{c^2 - a^2 v^2} = c \sqrt{1 - \frac{V^2} {c^2}}\]
Следовательно, единичный вектор скорости второго наблюдателя имеет вид
\[e'_0=(\frac 1 L, \frac v L, 0, 0)\]
Мы ищем вектор
\[e'_1=(A, B, 0, 0)\]
который ортогонален вектору $e'_0$. Для этого мы имеем
	\begin{equation}
c^2 A^2 - a^2 B^2 = -1
	\label{eq: length of vector, e1, 1}
	\end{equation}
	\begin{equation}
c^2 A \frac 1 L - a^2 B \frac v L = 0
	\label{eq: length of vector, e1, 2}
	\end{equation}
Мы получим из уравнения \eqref{eq: length of vector, e1, 2}
	\begin{equation}
A = \frac {a^2} {c^2} v B
	\label{eq: length of vector, e1, 3}
	\end{equation}
Мы подставим \eqref{eq: length of vector, e1, 3}
в \eqref{eq: length of vector, e1, 1} и получим
\[B^2 (\frac {a^4} {c^2} v^2 - a^2) = -1\] 
\[B = \frac 1 {a \sqrt{1 - \frac {V^2} {c^2}}}\]
Следовательно базис второго наблюдателя имеет вид
\[e'_0=(\frac 1 {c \sqrt{1 - \frac{V^2} {c^2}}}, \frac V {c a\sqrt{1 - \frac{V^2} {c^2}}}, 0, 0)\]
\[e'_1=( \frac V {c^2 \sqrt{1 - \frac {V^2} {c^2}}},
\frac 1 {a \sqrt{1 - \frac {V^2} {c^2}}}, 0, 0)\]
Теперь мы можем выразить $e'$ через $e$
\[e'_0= \frac 1 {\sqrt{1 - \frac {V^2} {c^2}}} e_0
+ \frac V c \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_1\]
\[e'_1= \frac V c \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_0
+ \frac 1 {\sqrt{1 - \frac{V^2} {c^2}}} e_1\] 


==> Geom.Object.Russian.tex <==
%auto-ignore
\def\texGeomObject{}
\ifx\PrintBook\Defined
				\chapter{Геометрический объект}
\fi

			\section{Метрико-аффинного многообразие}

В случае связности \xEqRef{0405.027}{eq: GLn connection form}
мы определим \AddIndex{форму кручение}{torsion form}
	\begin{equation}
T^a = d^2 x^a + \omega^a_b \wedge dx^b
	\label{eq: Torsion}
	\end{equation}
Из \xEqRef{0405.027}{eq: GLn connection form} следует
	\begin{equation}
\omega^a_b \wedge dx^b=(\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
	\label{eq: wedge connection}
	\end{equation}
Подставляя \eqref{eq: wedge connection} и \xEqRef{0405.027}{eq: anholonomity} в \eqref{eq: Torsion}
мы получим
	\begin{equation}
T^a=T^a_{cb}dx^c\wedge dx^b =
-c^a_{cb}dx^c\wedge dx^b + (\Gamma^a_{bc}-\Gamma^a_{cb})dx^c\wedge dx^b
\label{eq: Torsion 1}
	\end{equation}
где мы определили \AddIndex{тензор кручение}{torsion tensor}
	\begin{equation}
T^a_{cb} =
\Gamma^a_{bc}-\Gamma^a_{cb}-c^a_{cb}
\label{eq: Torsion coordinates}
	\end{equation}

Коммутатор вторых производных имеет вид
	\begin{equation}
u^\alpha_{;kl}-u^\alpha_{;lk}
=R^\alpha_{\beta lk}u^\beta
-T^p_{lk}u^\alpha_{;p}
	\label{eq: commutator second derivative}
	\end{equation}
Из \eqref{eq: commutator second derivative} следует, что
	\begin{equation}
	\label{eq: commutator second derivative of vector}
\xi^a_{;cb}-\xi^a_{;bc}
=R^a_{d bc}\xi^d
-T^p_{bc}\xi^a_{;p}
	\end{equation}

В римановом пространстве мы have metric tensor $g_{ij}$ и связность $\Gamma^k_{ij}$.
Одно из свойств риманова пространства - это симметрия связности и равенство нулю ковариантной производной
метрики. Это порождает тесную связь между метрикой и связностью.
However  связность is not necessarily symmetric
и ковариантная производная метрического тензора может быть отлична от 0.
В последнем случае мы вводим \AddIndex{неметричность}{nonmetricity}
	\begin{equation}
Q^{ij}_k=g^{ij}_{;k}=g^{ij}_{,k}+\Gamma^i_{pk}g^{pj}+\Gamma^j_{pk}g^{ip}
	\label{eq: Nonmetricity}
	\end{equation}

Так как производная метрического тензора не равна 0, мы не можем поднимать или опускать индекс
тензора внутри производной как мы это делаем в обычном римановом пространстве.
Теперь эта операция принимает следующий вид
\[a^i_{;k} = g^{ij} a_{j;k} + g^{ij}_{;k} a_j\]
Это равенство для метрического тензора принимает следующий вид
\[g^{ab}_{;k} = - g^{ai} g^{bj} g_{ij;k}\]

		\begin{definition}
Мы будем называть многообразие с кручением
и неметричностью
\AddIndex{метрико-аффинным многообразием}{metric-affine manifold} \citeBib{Mielke}.
		\qed  
		\end{definition}

Если мы изучаем подмногообразие $V_n$ многообразия $V_{n+m}$, мы видим, что имерсия порождает
связность $\Gamma^\alpha_{\beta\gamma}$, которая связана со связностью в многообразии соотношением
\[
\Gamma^\alpha_{\beta\gamma} e^l_\alpha =
\Gamma^l_{mk} e^m_\beta e^k_\gamma + \frac {\partial e^l_\beta} {\partial u^\gamma}
\]
Следовательно, не существует непрерывного вложения
пространства с кручением в риманово пространство.

			\section{Геометрический смысл кручения}

Предположим, что $a$ и $b$ - неколинеарные векторы в точке $A$ (см. фиг. \ref{fig:Torsion}).

%\begin{table}[h]
\begin{tabular}{l|r}
\begin{minipage}{160pt}
Мы проведём геодезическую $L_a$ через точку $A$, используя вектор $a$
как касательный вектор к $L_a$ в точке $A$.
Пусть $\tau$ - канонический параметр на $L_a$ и
\[\frac {dx^k}{d\tau}=a^k\]
Мы перенесём вектор $b$ вдоль геодезической $L_a$ из точки $A$
в точку $B$, определённую значением параметра $\tau=\rho>0$. Мы обозначим результат $b'$.
\end{minipage}
&
\begin{minipage}{160pt}
Мы проведём геодезическую $L_b$ через точку $A$, используя вектор $b$
как касательный вектор к $L_b$ в точке $A$.
Пусть $\varphi$ - канонический параметр на $L_b$ и
\[\frac {dx^k}{d\varphi}=b^k\]
Мы перенесём вектор $a$ вдоль геодезической $L_b$ из точки $A$
в точку $D$, определённую значением параметра $\varphi=\rho>0$. Мы обозначим результат $a'$.
\end{minipage}
\end{tabular}
%\end{table}

%\begin{table}[h]
\begin{tabular}{l|r}
\begin{minipage}{160pt}
Мы проведём геодезическую $L_{b'}$ через точку $B$, используя вектор $b'$
как касательный вектор к $L_{b'}$ в точке $B$.
Пусть $\varphi'$ - канонический параметр на $L_{b'}$ и 
\[\frac {dx^k}{d\varphi'}=b'^k\]
Мы определим точку $C$ на геодезической $L_{b'}$ значением параметра $\varphi'=\rho$
\end{minipage}
&
\begin{minipage}{160pt}
Мы проведём геодезическую $L_{a'}$ через точку $D$, используя вектор $a'$
как касательный вектор к $L_{a'}$ в точке $D$.
Пусть $\tau'$ - канонический параметр на $L_{a'}$ и 
\[\frac {dx^k}{d\tau'}=a'^k\]
Мы определим точку $E$ на геодезической $L_{a'}$ значением параметра $\tau'=\rho$
\end{minipage}
\end{tabular}
%\end{table}

Формально линии $AB$ и $DE$ так же, как линии $AD$ и $BC$, параллельны.
Длины отрезков $AB$ и $DE$ равны так же, как длины
отрезков $AD$ и $BC$ равны. Мы называем такую фигуру
\AddIndex{параллелограммом}{parallelogram}, построенным на векторах
$a$ и $b$ с вершиной в точке $A$.

		\begin{theorem}
Предположим $CBADE$ - параллелограм с вершиной в точке
$A$; тогда построенная фигура не будет замкнута \citeBib{torsion}.
Величина различия координат
точек $C$ и $E$ равна поверхностному интегралу кручения
над этим параллелограммом\footnote{Доказательство этого утверждения я нашёл в \citeBib{Shilov}}
\[\Delta_{CE}x^k=\iint T^k_{mn}dx^m \wedge dx^n \]
		\end{theorem}

	\begin{figure}
	\begin{center}
	\begin{picture}(150,150)
\put( 20, 25){ $A$ }
\put( 30, 65){ $a$ }
\put( 45, 50){ $b$ }
\put( 55, 130){ $B$ }
\put( 80, 135){ $b'$ }
\put( 155, 80){ $a'$ }
\put( 165, 150){ $C$ }
\put( 170, 40){ $D$ }
\put( 195, 135){ $E$ }
\put(-115, -65){\qbezier(150,100)(162,150)(185,190)}%AB
\put(35, 35){\vector(1,4){11}}%a
%\put(35, 35){\line(2, 5){36}}%AB
\put(-115, -65){\qbezier(185,190)(218,207)(283,210)}%BC
\put(70, 125){\vector(2,1){30}}%b'
%\put(70, 125){\line(5, 1){98}}%BC
\put(169, 145){\line(3, -2){18}}%CE
\put(-149, -154){\qbezier(320,212)(323,260)(336,287)}%DE
\put(171, 59){\vector(0,1){35}}%a'
%\put(174, 59){\line(1, 6){12.4}}%DE
\put(-149, -154){\qbezier(185,190)(208,206)(320,212)}%AD
\put(35, 35){\vector(3,2){30}}%b
%\put(35, 35){\line(6, 1){139}}%AD
	\end{picture}
	\caption{Meaning of Torsion}
	\label{fig:Torsion}
	\end{center}
	\end{figure}
		\begin{proof}
Мы можем найти приращение координаты $x^k$ вдоль геодезической в виде
	\begin{align*}
\Delta x^k&=\frac{dx^k}{d\tau}\tau+\frac 1 2 \frac{d^2 x^k}{d\tau^2}\tau^2+O(\tau^2)=\\
&=\frac{dx^k}{d\tau}\tau-\frac 1 2 \Gamma^k_{mn}\frac{dx^m}{d\tau} \frac{dx^n}{d\tau}\tau^2+O(\tau^2)
	\end{align*}
где $\tau$ - канонический параметр и мы вычисляем производные и компоненты
$\Gamma^k_{mn}$ в начальной точке. В частности 
	\[
\Delta_{AB} x^k=a^k\rho-\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2+O(\rho^2)
	\]
вдоль геодезической $L_a$ и
	\begin{equation}
\Delta_{BC} x^k=b'^k\rho-\frac 1 2 \Gamma^k_{mn}(B)b'^m b'^n\rho^2+O(\rho^2)
	\label{eq:Torsion_1}
	\end{equation}
вдоль геодезической $L_{b'}$. Здесь
	\begin{equation}
b'^k=b^k- \Gamma^k_{mn}(A)b^m dx^n+O(dx)
	\label{eq:Torsion_2}
	\end{equation}
результат параллельного переноса $b^k$ из $A$ в $B$ и
	\begin{equation}
dx^k=\Delta_{AB} x^k=a^k\rho
	\label{eq:Torsion_3}
	\end{equation}
с точностью до малой первого порядка. Подставляя
\eqref{eq:Torsion_3} в \eqref{eq:Torsion_2} и \eqref{eq:Torsion_2} в
\eqref{eq:Torsion_1}, мы получим
\[
\Delta_{BC} x^k=b^k \rho- \Gamma^k_{mn}(A)b^m a^n \rho^2
-\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2+O(\rho^2)
\]
Общее приращение координаты $x^K$ вдоль пути $ABC$ имеет вид
\[
\Delta_{ABC}x^k=\Delta_{AB} x^k+\Delta_{BC} x^k=
\]
	\begin{equation}
	\label{eq:Torsion_4}
=(a^k+b^k)\rho- \Gamma^k_{mn}(A)b^m a^n \rho^2-
	\end{equation}
\[
-\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2
-\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2+O(\rho^2)
\]

Аналогично общее приращение координаты $x^K$ вдоль пути $ADE$ имеет вид
\[
\Delta_{ADE}x^k=\Delta_{AD} x^k+\Delta_{DE} x^k=
\]
	\begin{equation}
	\label{eq:Torsion_5}
=(a^k+b^k)\rho- \Gamma^k_{mn}(A)a^m b^n \rho^2-
	\end{equation}
\[
-\frac 1 2 \Gamma^k_{mn}(D)a^m a^n\rho^2
-\frac 1 2 \Gamma^k_{mn}(A)b^m b^n\rho^2+O(\rho^2)
\]

Из \eqref{eq:Torsion_4} и \eqref{eq:Torsion_5} следует, что
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k=\]
\[= \Gamma^k_{mn}(A)b^m a^n\rho^2
+\underline{\frac 1 2 \Gamma^k_{mn}(B)b^m b^n\rho^2}_1
+\underline{\frac 1 2 \Gamma^k_{mn}(A)a^m a^n\rho^2}_2-\]
\[- \Gamma^k_{mn}(A)a^m b^n \rho^2
-\underline{\frac 1 2 \Gamma^k_{mn}(D)a^m a^n\rho^2}_2
-\underline{\frac 1 2 \Gamma^k_{mn}(A)b^m b^n\rho^2}_1+O(\rho^2)
\]
Для достаточно малого значения $\rho$ подчёркнутые слагаемые взаимно уничтожаются
и мы получаем интегральную сумму для выражения
\[
\Delta_{ADE}x^k-\Delta_{ABC}x^k=\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn})dx^m \wedge dx^n
\]

Однако недостаточно найти разность
\[\Delta_{ADE}x^k-\Delta_{ABC}x^k\]
чтобы найти разность координат точек $C$ и $E$.
Координаты могут быть неголономными и мы должны учесть, что
координаты вдоль замкнутого пути изменяются \xEqRef{0405.027}{eq: change of coordinate along a loop}
\[\Delta x^k=\oint_{ECBADE}dx^k=-\iint_\Sigma c^k_{mn}dx^m \wedge dx^n \]
где $c$ - объект неголономности.

Окончательно разность координат точек $C$ и $E$ имеет вид
\[\Delta_{CE}x^k=\Delta_{ADE}x^k-\Delta_{ABC}x^k+\Delta x^k=
\iint_\Sigma (\Gamma^k_{nm}- \Gamma^k_{mn}-c^k_{mn})dx^m \wedge dx^n\]
Используя \eqref{eq: Torsion coordinates}, мы доказали утверждение. 
		\end{proof}

			\section{Соотношение между связностью и метрикой}

Сейчас мы хотим найти, как мы можем выразить связность, если известны
метрика и кручение. Согласно определению
\[-Q_{kij}=g_{ij;k}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{jk}g_{pi}\]
\[-Q_{kij}=g_{ij,k}-\Gamma^p_{ik}g_{pj}-\Gamma^p_{kj}g_{pi}-S^p_{jk}g_{pi}\]
Перенесём производную $g$ и кручение в левую часть.
	\begin{equation}
g_{ij,k}+Q_{kij}-S^p_{jk}g_{pi}=\Gamma^p_{ik}g_{pj}+\Gamma^p_{kj}g_{pi}
	\label{eq: Connection1}
	\end{equation}
Меняя порядок индексов, мы запишем ещё два уравнения
	\begin{equation}
g_{jk,i}+Q_{ijk}-S^p_{ki}g_{pj}=\Gamma^p_{ji}g_{pk}+\Gamma^p_{ik}g_{pj}
	\label{eq: Connection2}
	\end{equation}
	\begin{equation}
g_{ki,j}+Q_{jki}-S^p_{ij}g_{pk}=\Gamma^p_{kj}g_{pi}+\Gamma^p_{ji}g_{pk}
	\label{eq: Connection3}
	\end{equation}
Если мы вычтем равенство \eqref{eq: Connection1} из суммы равенств
\eqref{eq: Connection2} и \eqref{eq: Connection1}, то мы получим
\[
g_{ki,j}+g_{jk,i}-g_{ij,k}+Q_{ijk}+Q_{jki}-Q_{kij}
-S^p_{ij}g_{pk}-S^p_{ki}g_{pj}+S^p_{jk}g_{pi}=2\Gamma^p_{ji}g_{pk}
\]
Окончательно мы получаем
\[
\Gamma^p_{ji}=\frac 1 2 g^{pk}
(g_{ki,j}+g_{jk,i}-g_{ij,k}+Q_{ijk}+Q_{jki}-Q_{kij}
-S^r_{ij}g_{rk}-S^r_{ki}g_{rj}+S^r_{jk}g_{ri})
\]


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index{texLinearMap}%1%1
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index{texPolymodule}%2%66
   {$(2)$\hyph векторное пространство}%
   {(2)-vector space}%
\Index{texBundleRelation}%2%122
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index{texBiring}%A%2
   {$(^{\gi a}_{\gi b})$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index{texBiring}%A%34
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index{texCalculus}%A%67
   {$A$\Hyph значная функция}%
   {A valued function}%
\SetIndexSpace%
\Index{texBiring}%C%3
   {\subs строка матрицы}%
   {c row}%
\Index{texVectorSpace}%C%5
   {\CR матричная группа}%
   {cr-matrix group}%
\Index{texBiring}%C%6
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index{texBiring}%C%7
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index{texBiring}%C%8
   {\CR степень}%
   {cr power}%
\Index{texVectorSpace}%C%9
   {\crd векторное пространство}%
   {crd vector space}%
\Index{texBiring}%C%10
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index{texVectorSpace}%D%11
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index{texVectorSpace}%D%12
   {\dcr вектор}%
   {dcr vector}%
\Index{texVectorSpace}%D%13
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index{texVectorSpace}%D%14
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index{texVectorSpace}%D%15
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index{texVectorSpace}%D%55
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index{texVectorSpace}%D%17
   {\drc базис}%
   {}%
\SubIndex{texVectorSpace}%4%
   {в векторном пространстве}%
   {drc basis, vector space}%
\SubIndex{texVectorSpace}%5%
   {в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index{texVectorSpace}%D%18
   {\drc вектор}%
   {drc vector}%
\Index{texVectorSpace}%D%19
   {\drc векторное пространство}%
   {drc vector space}%
\Index{texVectorSpace}%D%20
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index{texCalculus}%D%46
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index{texVectorSpace}%D%83
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index{texVectorSpace}%D%87
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Index{texVectorSpace}%D%23
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index{texVectorSpace}%D%114
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index{texDrcMorphism}%D%25
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index{texVectorSpace}%D%27
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index{texVectorSpace}%D%26
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index{texCalculus}%D%96
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\SetIndexSpace%
\Index{texELie}%E%28
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index{texDiffEq}%E%29
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index{texRefernceFrame}%G%205
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index{texTypeBasis}%G%30
   {\Gbasis}%
   {G-basis}%
\Index{texTypeBasis}%G%31
   {\Gcoords ы}%
   {G-coordinates}%
\Index{texTypeBasis}%G%32
   {\Gspace о}%
   {GSpace}%
\Index{texBasis}%G%267
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index{texBasis}%G%270
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index{texBasis}%G%271
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index{texPolymodule}%N%231
   {$(n)$\hyph векторное пространство}%
   {(n)-vector space}%
\Index{texBundleRelation}%N%218
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index{texBiring}%R%35
   {\sups строка матрицы}%
   {r row}%
\Index{texVectorSpace}%R%36
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index{texVectorSpace}%R%37
   {\RC главный минор}%
   {RC-major minor}%
\Index{texBiring}%R%38
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index{texVectorSpace}%R%39
   {\RC матричная группа}%
   {rc-matrix group}%
\Index{texVectorSpace}%R%40
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index{texBiring}%R%41
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index{texBiring}%R%42
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index{texVectorSpace}%R%43
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index{texBiring}%R%44
   {\RC степень}%
   {rc power}%
\Index{texVectorSpace}%R%45
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index{texVectorSpace}%R%213
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index{texBiring}%R%47
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index{texDrcMorphism}%S%314
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index{texLinearMap}%S%48
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index{texVectorSpace}%S%217
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index{texVectorSpace}%S%216
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index{texTstarRepresentation}%S%49
   {\sT сдвиг}%
   {starT shift}%
\Index{texFiberedGroup}%S%50
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\Index{texTstarMorphism}%S%160
   {\sT представление $\mathfrakl{F}$\Hyph алгебры $A$ в множестве $M$}%
   {starT representation of algebra}%
\Index{texFiberedAlgebra}%S%162
   {\sT представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index{texFiberedGroup}%S%163
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index{texTstarMorphism}%S%308
   {\sT преобразование}%
   {starT transformation}%
\Index{texFiberedAlgebra}%S%167
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\SubIndex{}%71%
   {невырожденное}%
   {nonsingular transformation of bundle}%
\SetIndexSpace%
\Index{texVectorSpace}%T%51
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index{texVectorSpace}%T%52
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index{texFiberedGroup}%T%316
   {\Ts представление расслоенной группы}%
   {Tstar representation of fibered group}%
\Index{texTstarRepresentation}%T%53
   {\Ts сдвиг}%
   {Tstar shift}%
\Index{texTstarMorphism}%T%301
   {\Ts представление $\mathfrakl{F}$\Hyph алгебры $A$ в множестве $M$}%
   {Tstar representation of algebra}%
\Index{texFiberedAlgebra}%T%321
   {\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index{texTstarMorphism}%T%309
   {\Ts преобразование}%
   {Tstar transformation}%
\Index{texFiberedAlgebra}%T%327
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\SetIndexSpace%
\Index{texNewton}%V%54
   {vector potential}%
   {vector potential}%
\SetIndexSpace%
\Index{texAffine}%А%56
   {автопараллельная кривая}%
   {auto parallel line}%
\Index{texDrcBasis}%А%57
   {активное \sT представление}%
   {active representation, vector space}%
\Index{texBasis}%А%262
   {активное представление}%
   {active representation}%
\Index{texBasis}%А%263
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index{texLie}%А%58
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\SubIndex{texLie}%9%
   {определённая слева}%
   {left defined algebra Lie}%
\SubIndex{texLie}%10%
   {определённая справа}%
   {right defined algebra Lie}%
\Index{texBiring}%А%59
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index{texFiberedGroup}%А%60
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index{texBundleRelation}%А%156
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index{texFiberedAlgebra}%А%61
   {арность операции}%
   {arity of operation}%
\Index{texBasis}%А%277
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index{texBasis}%А%275
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index{texBundle}%Б%172
   {база отображения}%
   {base of map}%
\Index{texBundleRelation}%Б%233
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index{texTypeBasis}%Б%16
   {базис}%
   {}%
\SubIndex{texTypeBasis}%1%
   {аффинный}%
   {Affine Basis}%
\SubIndex{texTypeBasis}%2%
   {ортонормальный}%
   {Orthonornal Basis}%
\SubIndex{texTypeBasis}%3%
   {центро-аффинный}%
   {Central Affine Basis}%
\Index{texBasis}%Б%266
   {базис векторного пространства}%
   {Basis}%
\Index{texLieRepresentation}%Б%62
   {базовый вектор}%
   {}%
\SubIndex{texLieRepresentation}%11%
   {\sT представления}%
   {basis vector of starT representation}%
\SubIndex{texLieRepresentation}%12%
   {\Ts представления}%
   {basis vector of Tstar representation}%
\Index{texLie}%Б%63
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index{texFiberedMorphism}%Б%351
   {башня расслоений}%
   {tower of bundles}%
\Index{texLieRepresentation}%Б%64
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index{texBiring}%Б%65
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index{texPolymodule}%В%230
   {($D_1\RCstar$, ..., $D_n\RCstar$)\hyph векторное пространство}%
   {(d1rc,dnrc)-vector space}%
\Index{texPolymodule}%В%229
   {($S\star$, $\star T$)\hyph векторное пространство}%
   {(Sstar,starT)-vector space}%
\Index{texDiffProperty}%В%69
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index{texRepresentation}%В%261
   {вектор\hyph столбец}%
   {column vector}%
\Index{texFiberedAlgebra}%В%70
   {векторное расслоение}%
   {vector bundle}%
\Index{texRepresentation}%В%260
   {вектор\hyph строка}%
   {row vector}%
\Index{texDiffEq}%В%71
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index{texNewton}%В%72
   {второй закон Ньютона}%
   {Second Newton law}%
\SetIndexSpace%
\Index{texDrcBasis}%Г%73
   {геометрический объект}%
   {}%
\SubIndex{texDrcBasis}%13%
   {в координатном представлении,	определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\SubIndex{texDrcBasis}%14%
   {определённый в векторном пространстве}%
   {geometrical object, vector space}%
\SubIndex{texDrcBasis}%15%
   {типа $A$}%
   {geometrical object of type A, vector space}%
\Index{texBasis}%Г%290
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index{texBasis}%Г%288
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index{texBasis}%Г%293
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index{texRefernceFrame}%Г%74
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index{texRefernceFrame}%Г%195
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index{texFiberedAlgebra}%Г%75
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index{texFiberedGroup}%Г%76
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index{texTypeBasis}%Г%77
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%274
   {группа аффинных преобразований}%
   {AffineTransformationGroup}%
\Index{texBasis}%Г%264
   {группа симметрии}%
   {symmetry group}%
\Index{texDrcBasis}%Г%78
   {группа симметрии}%
   {SymmetryGroup}%
\Index{texTstarRepresentation}%Г%344
   {группа стабилизации}%
   {stability group}%
\Index{texGroupRing}%Г%79
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index{}%Д%283
   {движение на многообразии базисов}%
   {movement transformation}%
\Index{texBundle}%Д%331
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index{texBundle}%Д%357
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%176
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Index{texCartesian}%Д%180
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index{texCartesian}%Д%181
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index{texBundleRelation}%Д%113
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index{texBundleRelation}%Д%227
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index{texCalculus}%Д%105
   {дифференциал отображения нормированного \drc векторного пространства в нормированное тело}%
   {differential, drc vector space to skew field}%
\Index{texCalculus}%Д%99
   {дифференцируемая функция \drc векторного пространства в тело $D$ }%
   {differentiable functions, drc vector space to skew field}%
\SetIndexSpace%
\Index{texDrcMorphism}%З%312
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index{texVectorSpace}%З%310
   {закон ассоциативности для \Ts векторного пространства}%
   {associative law, Tstar vector space}%
\Index{texTstarRepresentation}%З%80
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for Tstar covariant representation}%
\Index{texLinearMap}%З%311
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index{texBundleRelation}%З%155
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index{texVectorSpace}%З%81
   {закон дистрибутивности}%
   {}%
\SubIndex{texVectorSpace}%20%
   {\Ts векторное пространство}%
   {distributive law, Tstar vector space}%
\Index{texVectorSpace}%З%82
   {закон унитарности}%
   {}%
\SubIndex{texVectorSpace}%21%
   {для \Ts векторного пространства}%
   {unitarity law, Tstar vector space}%
\SetIndexSpace%
\Index{texFiberedAlgebra}%И%84
   {изоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {isomorphism of fibered F-algebras}%
\Index{texLinearLie}%И%85
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index{texHomotopy}%К%4
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index{texBundleRelation}%К%111
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index{texBundleRelation}%К%112
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index{texBasis}%К%278
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index{texBasis}%К%284
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index{texFiberedGroup}%К%318
   {ковариантное \Ts представление расслоенной группы}%
   {Tstar covariant representation of fibered group}%
\Index{texBundleRelation}%К%228
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index{texBundle}%К%332
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index{texFiberedGroup}%К%317
   {контравариантное \Ts представление расслоенной группы}%
   {Tstar contravariant representation of fibered group}%
\Index{texVectorSpace}%К%21
   {координатная матрица}%
   {}%
\SubIndex{texVectorSpace}%6%
   {вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\SubIndex{texVectorSpace}%7%
   {множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\SubIndex{texVectorSpace}%8%
   {множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index{texRefernceFrame}%К%86
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index{texBasis}%К%285
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index{texDrcBasis}%К%88
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%287
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index{texBasis}%К%286
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%89
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index{texVectorSpace}%К%22
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index{texDrcBasis}%К%90
   {координаты геометрического объекта}%
   {}%
\SubIndex{texDrcBasis}%22%
   {в векторном пространстве}%
   {coordinates of geometrical object, vector space}%
\SubIndex{texDrcBasis}%23%
   {в координатном векторном пространстве}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texBasis}%К%291
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index{texBasis}%К%289
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index{texVectorSpace}%К%91
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index{texVectorSpace}%К%92
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index{texDrcBasis}%К%93
   {координаты представления}%
   {coordinates of representation}%
\Index{texBasis}%К%265
   {координаты представления}%
   {coordinates of representation}%
\Index{texAffine}%К%94
   {кривизна Картана}%
   {Cartan curvature}%
\SetIndexSpace%
\Index{texVectorSpace}%Л%98
   {левое векторное пространство}%
   {left vector space}%
\Index{texLie}%Л%101
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index{texRepresentation}%Л%247
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation}%
\Index{texRepresentation}%Л%249
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation}%
\Index{texTstarMorphism}%Л%302
   {левостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {left-side representation of algebra}%
\Index{texRepresentation}%Л%244
   {левостороннее представление группы}%
   {left-side representation of group}%
\Index{texFiberedAlgebra}%Л%322
   {левостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%Л%164
   {левостороннее преобразование}%
   {left-side transformation}%
\Index{texFiberedAlgebra}%Л%328
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index{texLie}%Л%103
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index{texVectorSpace}%Л%214
   {левый модуль}%
   {left module}%
\Index{texTstarRepresentation}%Л%108
   {левый сдвиг}%
   {left shift}%
\Index{texRepresentation}%Л%251
   {левый сдвиг на группе}%
   {left shift, group}%
\Index{texFiberedGroup}%Л%109
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index{texRepresentation}%Л%240
   {линейное представление группы}%
   {linear representation of group}%
\Index{texBundle}%Л%116
   {лифт отображения}%
   {lift of map}%
\Index{texBundleRelation}%Л%232
   {лифт соответствия}%
   {lift of correspondence}%
\Index{texRefernceFrame}%Л%117
   {локальная система отсчёта}%
   {local reference frame}%
\SetIndexSpace%
\Index{texTstarRepresentation}%М%343
   {малая группа}%
   {little group}%
\Index{texDrcMorphism}%М%118
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index{texGeomObject}%М%119
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index{texDrcBasis}%М%120
   {многообразие базисов}%
   {}%
\SubIndex{texDrcBasis}%24%
   {\drc векторного пространства}%
   {basis manifold of vector space}%
\SubIndex{texTypeBasis}%25%
   {аффинного пространства}%
   {Basis Manifold, Affine Space}%
\SubIndex{texTypeBasis}%26%
   {евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\SubIndex{texTypeBasis}%27%
   {центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texBasis}%М%276
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index{texBasis}%М%268
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index{texBasis}%М%282
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index{texBasis}%М%280
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index{texDrcReferenceFrame}%М%123
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index{texFiberedMorphism}%М%355
   {морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of fibered F algebra}%
\Index{texTstarMorphism}%М%298
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of F algebra}%
\Index{texTstarMorphism}%М%300
   {морфизм \Ts представлений $\mathfrak{F}$\Hyph алгебры в $\mathfrak{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index{texTstarMorphism}%М%307
   {морфизм \Ts представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index{texFiberedMorphism}%М%356
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index{texVectorSpace}%Н%124
   {невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index{texRepresentation}%Н%241
   {невырожденное \Ts преобразование}%
   {nonsingular transformation}%
\Index{texRefernceFrame}%Н%125
   {неголономная координата}%
   {anholonomic coordinate}%
\Index{texRefernceFrame}%Н%126
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index{texRefernceFrame}%Н%127
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index{texRefernceFrame}%Н%110
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index{texGeomObject}%Н%128
   {неметричность}%
   {nonmetricity}%
\Index{texBundleRelation}%Н%339
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index{texCalculus}%Н%97
   {норма на \drc векторном пространстве}%
   {norm on drc vector space}%
\Index{texCalculus}%Н%100
   {норма на теле}%
   {absolute value on skew field}%
\Index{texCalculus}%Н%102
   {нормированное тело}%
   {valued skew field}%
\Index{texCalculus}%Н%104
   {нормированным \drc векторное пространство}%
   {normed drc vector space}%
\SetIndexSpace%
\Index{texBundleRelation}%О%121
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index{texBundleRelation}%О%115
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index{texBiring}%О%129
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index{texRefernceFrame}%О%130
   {объект неголономности}%
   {anholonomity object}%
\Index{texTstarRepresentation}%О%131
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texRepresentation}%О%259
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index{texFiberedGroup}%О%132
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index{texTstarMorphism}%О%303
   {однотранзитивное представление алгебры $A$}%
   {single transitive representation of algebra}%
\Index{texRepresentation}%О%258
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index{texFiberedAlgebra}%О%323
   {однотранзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index{texFiberedAlgebra}%О%133
   {операция на расслоении}%
   {operation on bundle}%
\Index{texBiring}%О%134
   {определитель матрицы}%
   {determinant}%
\Index{texTstarRepresentation}%О%135
   {орбита \Ts представления группы}%
   {orbit of representation of group}%
\Index{texRepresentation}%О%253
   {орбита представления группы}%
   {orbit of representation of group}%
\Index{texFiberedGroup}%О%136
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index{texBasis}%О%281
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index{texTidal}%О%137
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index{texDrcReferenceFrame}%О%138
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\SetIndexSpace%
\Index{texGeomObject}%П%139
   {параллелограмм}%
   {parallelogram}%
\Index{texTstarRepresentation}%П%140
   {парные представления группы}%
   {twin representations of group}%
\Index{texFiberedGroup}%П%319
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index{texLinearMap}%П%320
   {парные представления тела}%
   {twin representations of skew field}%
\Index{texDrcBasis}%П%141
   {пассивное \Ts представление}%
   {passive representation}%
\Index{texBasis}%П%273
   {пассивное представление}%
   {passive representation}%
\Index{texBasis}%П%272
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index{texNewton}%П%142
   {первый закон Ньютона}%
   {First Newton law}%
\Index{texAffine}%П%143
   {перенос Картана}%
   {Cartan transport}%
\Index{texAffine}%П%144
   {перенос Френе}%
   {Frenet transport}%
\Index{texBundle}%П%220
   {подрасслоение}%
   {subbundle}%
\Index{texNewton}%П%146
   {потенциальная энергия}%
   {potential energy}%
\Index{texVectorSpace}%П%149
   {правое векторное пространство}%
   {right vector space}%
\Index{texLie}%П%151
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index{texRepresentation}%П%248
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation}%
\Index{texRepresentation}%П%250
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation}%
\Index{texTstarMorphism}%П%304
   {правостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в множестве $M$}%
   {right-side representation of algebra}%
\Index{texRepresentation}%П%245
   {правостороннее представление группы}%
   {right-side representation of group}%
\Index{texFiberedAlgebra}%П%324
   {правостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index{texTstarMorphism}%П%242
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texRepresentation}%П%243
   {правостороннее преобразование}%
   {right-side transformation}%
\Index{texLie}%П%153
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index{texVectorSpace}%П%215
   {правый модуль}%
   {right module}%
\Index{texTstarRepresentation}%П%158
   {правый сдвиг}%
   {right shift}%
\Index{texRepresentation}%П%252
   {правый сдвиг на группе}%
   {right shift, group}%
\Index{texBundleRelation}%П%342
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index{texBundleRelation}%П%335
   {предел фильтра}%
   {limit of filter}%
\Index{texBundleRelation}%П%334
   {предельное множество фильтра}%
   {limit set of filter}%
\Index{texBasis}%П%292
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texDrcBasis}%П%159
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index{texRepresentation}%П%246
   {представление группы}%
   {representation of group}%
\Index{texTstarRepresentation}%П%161
   {представление группы}%
   {}%
\SubIndex{texDrcBasis}%38%
   {\drc линейное \sT}%
   {linear representation of group}%
\SubIndex{texDrcBasis}%39%
   {\rcd}%
   {rcd linear representation of group}%
\SubIndex{texTstarRepresentation}%40%
   {\sT}%
   {starT representation of group}%
\SubIndex{texTstarRepresentation}%41%
   {\Ts}%
   {Tstar representation of group}%
\SubIndex{texTstarRepresentation}%42%
   {ковариантное \Ts}%
   {Tstar covariant representation of group}%
\SubIndex{texTstarRepresentation}%43%
   {контравариантное \Ts}%
   {Tstar contravariant representation of group}%
\SubIndex{texTstarRepresentation}%44%
   {эффективное}%
   {effective representation of group}%
\Index{texRefernceFrame}%П%165
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index{texTstarMorphism}%П%313
   {преобразование множества}%
   {transformation of set}%
\Index{texDrcBasis}%П%166
   {преобразование на многообразии базисов}%
   {}%
\SubIndex{texDrcBasis}%62%
   {активное}%
   {active transformation, vector space}%
\SubIndex{texTypeBasis}%63%
   {аффинное}%
   {affine transformation}%
\SubIndex{texTypeBasis}%64%
   {движение}%
   {movement transformation}%
\SubIndex{texTypeBasis}%65%
   {квазиаффинное}%
   {quasi affine transformation}%
\SubIndex{texTypeBasis}%66%
   {квазидвижение}%
   {quasi movement}%
\SubIndex{texDrcBasis}%67%
   {пассивное}%
   {passive transformation, vector space}%
\Index{texFiberedAlgebra}%П%329
   {преобразование расслоения}%
   {transformation of bundle}%
\Index{texCartesian}%П%221
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index{texCartesian}%П%222
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index{texBundleRelation,texBundleRelation}%П%225
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index{texBundleRelation}%П%226
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index{texBiring}%П%168
   {приводимое бикольцо}%
   {reducible biring}%
\Index{texBiring}%П%169
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index{texBiring}%П%170
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index{texDrcBasis}%П%171
   {принцип инвариантности}%
   {invariance principle}%
\Index{texBasis}%П%296
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index{texBundleRelation}%П%235
   {продолжение соответствия}%
   {extension of correspondence}%
\Index{texBundle}%П%354
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index{texDrcBasis}%П%173
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index{texBasis}%П%295
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index{texTstarMorphism}%П%299
   {произведение морфизмов \Ts представлений $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index{texBundleRelation}%П%154
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index{texBundleRelation}%П%188
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\SubIndex{texVectorSpace}%74%
   {\drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\SubIndex{texVectorSpace}%75%
   {\rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index{texAffine}%П%174
   {производная Картана}%
   {Cartan derivative}%
\Index{texDiffProperty}%П%175
   {производная Ли}%
   {Lie derivative}%
\SubIndex{texDiffProperty}%72%
   {метрики}%
   {Lie derivative of metric}%
\SubIndex{texDiffProperty}%73%
   {связности}%
   {Lie derivative of connection}%
\Index{texTstarRepresentation}%П%352
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index{texCartesian}%П%333
   {пространство отображений}%
   {mapping space}%
\Index{texBundleRelation}%П%236
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index{texLieRepresentation}%П%177
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index{texTstarRepresentation}%П%178
   {прямое произведение \Ts представлений группы}%
   {direct product of representations of group}%
\Index{texRepresentation}%П%254
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index{texFiberedGroup}%П%179
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index{texRefernceFrame}%П%182
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index{texVectorSpace}%Р%183
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index{texFiberedMorphism}%Р%350
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index{texFiberedMorphism}%Р%349
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index{texFiberedAlgebra}%Р%184
   {расслоенная $\mathfrak{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index{texFiberedAlgebra}%Р%186
   {расслоенная $\mathfrak{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index{texFiberedAlgebra}%Р%185
   {расслоенная группа}%
   {fibered group}%
\Index{texFiberedMorphism}%Р%347
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index{texFiberedMorphism}%Р%346
   {расслоенная малая группа}%
   {fibered little group}%
\Index{texBundleRelation}%Р%145
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index{texBundleRelation}%Р%237
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index{texBundleRelation}%Р%238
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index{texFiberedAlgebra}%Р%187
   {расслоенное кольцо}%
   {fibered ring}%
\Index{texBundle}%Р%219
   {расслоенное подмножество}%
   {fibered subset}%
\Index{texBundleRelation}%Р%224
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index{texBundleRelation}%Р%330
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index{texBundleRelation}%Р%223
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index{texFiberedMorphism}%Р%337
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index{texBundle}%Р%353
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index{texFiberedMorphism}%Р%338
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index{texBundleRelation}%Р%157
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\SetIndexSpace%
\Index{texTstarRepresentation}%С%345
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index{texFiberedMorphism}%С%348
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index{texAffine}%С%189
   {связность Картана}%
   {Cartan connection}%
\Index{texAffine}%С%190
   {символ Картана}%
   {Cartan symbol}%
\Index{texBiring}%С%191
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index{texBundleRelation}%С%148
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index{texGenRelativity}%С%192
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index{texVectorSpace}%С%193
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index{texRefernceFrame}%С%194
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index{texNewton}%С%196
   {скалярный потенциал}%
   {scalar potential}%
\Index{texTidal}%С%197
   {скорость отклонения}%
   {speed of deviation}%
\Index{texBundleRelation}%С%297
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index{texBundleRelation}%С%340
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index{texBiring}%С%198
   {стандартное представление матрицы}%
   {Standard representation}%
\Index{texDrcBasis}%С%199
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBasis}%С%269
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index{texBundleRelation}%С%234
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index{texLinearMap}%С%200
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index{texDrcBasis}%С%201
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index{texBasis}%С%294
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index{texGeomObject}%Т%95
   {тензор кручения}%
   {torsion tensor}%
\Index{texNewton}%Т%202
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index{texLie}%Т%203
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index{texVectorSpace}%Т%204
   {тип векторного пространства}%
   {vector space type}%
\Index{texCalculus}%Т%152
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index{texCalculus}%Т%33
   {топологическое тело}%
   {topological skew field}%
\Index{texBundleRelation}%Т%147
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index{texTstarMorphism}%Т%305
   {транзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index{texRepresentation}%Т%257
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index{texFiberedAlgebra}%Т%325
   {транзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index{texDiffProperty}%У%206
   {уравнение Килинга}%
   {Killing equation}%
\Index{texDiffProperty}%У%207
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index{texBiring}%У%208
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index{texFiberedMorphism}%Ф%336
   {фактор расслоение}%
   {quotient bundle}%
\Index{texBundleRelation}%Ф%341
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index{texGeomObject}%Ф%239
   {форма кручение}%
   {torsion form}%
\Index{texCalculus}%Ф%150
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index{texCalculus}%Ф%68
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index{texBasis}%Ц%279
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index{texCalculus}%Ч%106
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, skew field}%
\Index{texCalculus}%Ч%107
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping with respect to variable, drc vector space}%
\SetIndexSpace%
\Index{texAffine}%Э%209
   {экстремальная кривая}%
   {extreme line}%
\Index{texTstarMorphism}%Э%306
   {эффективное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index{texRepresentation}%Э%256
   {эффективное представление группы}%
   {effective representation of group}%
\Index{texFiberedAlgebra}%Э%326
   {эффективное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index{texFiberedGroup}%Э%315
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index{texVectorSpace}%Э%210
   {эффективное представление тела}%
   {effective representation of skew field}%
\SetIndexSpace%
\Index{texTstarRepresentation}%Я%211
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of representation of group}%
\Index{texRepresentation}%Я%255
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index{texFiberedGroup}%Я%212
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%

\CloseIndex


==> Intro.Russian.tex <==
%auto-ignore
\def\texIntro{}

\ifx\PrintBook\Defined
				\chapter{Введение}
			\section{Об этой книге}
			\label{section: About This Book}

Sometimes is very hard to give name for book that you want to write.
Even you wrote it the whole life. And may be for this reason.
The way is not finished. However I feel it is time to share with people
my discoveries. Only future will tell which parts of this research
will be useful.
This book starts from изучения геометрического объекта, turns to
reference frame in physics, then suddenly changes its course
to learn metric affine manifolds.

Since Einstein introduced general relativity, the close relation between geometry
and physics became a reality. At the same time, quantum mechanics introduced new concepts that
contradicted a tradition established during centuries.
All together, this meant that we need new geometrical concepts that will become part
of the language of quantum mechanics.
This is the reason for returning to the beginning.

The whole my life was dedicated to solve one of the greatest
mysteries that I met in the beginning of my life. When I learned
general relativity and quantum mechanics I felt that language of
quantum mechanics is not adequate to phenomenon that it observes.
I mean the geometry.

Я посвятил главу \ref{chapter: Space and Time in Physics}
небольшому сочинению, написанному мной, когда я был молод.\footnote{Unfortunately
some references are lost. If somebody recognize
familiar text, I will appreciate if he let me know exactly reference}
\fi

\ifx\texPrefaceTorsion\Defined
\section{Torsion}

Тесная связь между метрическим тензором и связностью является
основой римановой геометрии.
В то же время, связность и метрика, как любой геометрический объект, являются объектом измерения.
When we study the general relativity equation, we introduce the lagrangian where
the metric tensor and the connection are independent. Later on, we discover that the connection
is symmetric and find dependence between connection and metric tensor. One of the
reasons is in the simplicity of the lagrangian.

\ifx\PrintBook\Defined
Глава \ref{chapter: General Relativistic Field Equations}
формально завершает книгу, хотя исторически она отображает
исследование, с которого начался определённый этап моей жизни.
В основу уравнений, выведенных в этой главе, было положено
непосредственное объединение двух лагранжианов: гравитационного
и квантового полей.
Повидимому столь прямолинейный подход
послужил причиной неудачи. Любая попытка решить уравнения
\eqref{eq: Field}, \eqref{eq: Einstein},
\eqref{eq: Cartan} и
\eqref{eq: Maxwell} приводит к тому,
что эта системв распадается на уравнение Эйнштейна и
уравнение поля, которые независимы.

Последующее развитие физики показало, что объединение общей теории
относительности и квантовой механики требует более мощных методов.
Основные направления на сегодняшний день можно разделить на теорию
струн и петлевую теорию гравитации.

Однако несмотря на неудачу, анализ полученных уравнений очень важен.
\fi

Analysis of quantum field theory shows that either
symmetry связности либо dependence связности и метрики may be broken, 
поскольку неизбежны ошибки измерения.
As we expected this assumption leads particularly to space with torsion and nonzero covariant derivative
метрического тензора.
We call the affine connected manifold with metric tensor
the metric-affine manifold \citeBib{Mielke}.

Метрико-аффинное многообразие появляется в разных физических приложениях.
Очень важно понять какова геометрия этого пространства,
как кручение может влиять на физические процессы.
Именно поэтому небольшая группа физиков продолжает изучать теорию
гравитации с кручением
\citeBib{Mielke,Obukhov,Sardanashvily,Gauge,Neeman}.

Independence of metric tensor и связности allows us to see which object is responsible for different
phenomenon in geometry и therefore in physics.

In particular мы have two different definitions геодезической в Riemann многообразие.
Мы можем рассматривать геодезическую либо как кривую экстремальной длины
(соответствующую кривую мы называем экстремальной),
либо как кривую, вдоль которой касательный вектор переносится параллельно, оставаясь
касательным к кривой
(соответствующую кривую мы называем автопараллельной).
Nonmetricity means that parallel transport does not conserve a length of vector and an angle between
vectors. This leads to a difference between
definitions автопараллельной и экстремальной кривых (\citeBib{torsion} и
section \ref{section: Line with extreme length})
and to a change in the expression of the Frenet transport.
Изменение геометрии influences second Newton law which мы study in section \ref{NewtonLaw}.
I show in theorems \ref{theorem: LengthTangentVector} и \ref{theorem: First Newton law} 
that free falling particle chooses an extreme line transporting
its momentum along trajectory without change.

Форма второго закона Ньютона зависит от выбора формы потенциала.
В случае скалярного потенциала
второй закон Ньютона holds the relationship between force, mass and acceleration.
В случае векторного потенциала
анализ of motion in a gravitational field shows that the field-strength tensor
depends on the derivative of the metric tensor.

Nonmetricity dramatically changes law how orthogonal frame moves in space.
However изучение of parallel transport in space с неметричностью allows us
ввести перенос Картана and an introduction of the connection compatible with the metric tensor
(section \ref{section: Cartan Transport}). Перенос Картана
holds базис orthonormal and this makes it valuable tool
in dynamics (section \ref{NewtonLaw})
because the observer uses an orthonormal frame as his measurement tool.
The dynamics of a particle follows to the Cartan transport.
The question arises from this conclusion.
We can change the connection as we show above.
%or we can change the metric tensor as is shown
%in  such way that the parallel transport conserves
%the metric tensor\footnote{I am not agree with conclussion in paper \cite{Hehl},
%however this paper shows way how to find the metric tensor compatible with connection}.
Why we need to learn manifolds with an arbitrary connection and the metric tensor?
First of all, the learning of the метрико-аффинное многообразие shows why everything
works well in the Riemann многообразие and what changes in a general case.
Also physical constraints that appear in a model may lead to appearance of a неметричности
\citeBib{Gauge,Megged,gr-qc-9604027}.
Because the перенос Картана is the natural mechanism to conserve orthogonality
we expect that we will interpret a deviation of the test particle from the extreme line as
a result of an external to this particle
force\footnote{For instance if we extend the definition \eqref{eq: potential force} of a force
to a general case \eqref{eq: Newton} we can interpret a deviation of a charged particle
in electromagnetic field as result of the force
\[\ F^j=\frac e {cu^0} g^{ij} F_{li} u^l\]
The same way we can interpret a deviation of the auto parallel line as the force
\[F^i=-\frac {m c} {u^0} \Gamma(C)^i_{kl}u^ku^l\]
I remind that the символ Картана is the tensor}.
In this case the difference between two types of a transport
becomes measurable and meaningful. Otherwise another type
of a transport и неметричность не наблюдаемы и мы можем пользоваться
только переносом, совместимым с метрикой.

I see here one more opportunity. As follows from the paper \citeBib{Megged}
the torsion may depend on quantum properties of matter.
However the torsion is the part of the connection. This means that the connection may
also depend on quantum properties of matter. This may lead to breaking of
the перенос Картана. However this opportunity demands additional research.


The effects of torsion and неметричности are cumulative.
They may be small but measurable. We can observe their effects not only in strong
fields like black hole or Big Bang but in regular conditions
as well.
Studying geometry and dynamics of point particle gives us a way to test this point of view.
There is mind to test this theory in condition when spin of quantum field is accumulated.
We can test a deviation from second Newton law or measure torsion by observing
the movement of 2 different particles.

To test if the spacetime has the torsion we
can test the opportunity to build a parallelogram in spacetime. 
We can conduct such test in strong electromagnetic field.
We can get 2 particles or 2 photons that start their movement from the same point
and using a mirror to force them to move along opposite sides of the parallelogram.
We can start this test when we do not have electromagnetic field and then repeat it in its presence.
Если particles meet in the same place or we have the same interference then we have
torsion equal $0$ in this thread.
In particular, the torsion may influence the behavior of virtual particles.

To test if the spacetime has неметричность we
can measure a deviation of an extreme line
from an auto parallel line or
a deviation of unit vector of speed from its parallel transport.
\fi

\ifx\texPrefaceRefernceFrame\Defined
\section{Геометрический объект и принцип инвариантности}

\ifx\PrintBook\Defined
Разделы \ref{section: Basis in Vector Space}
и \ref{section: Geometrical Object of Vector Space}
was written under the great influence of the book \citeBib{Rashevsky}.
The studying of a homogenous space of a group of symmetry of a vector space
leads us to the definition базиса of this space. Многообразие базисов - это множество
базисов of particular vector space and is an example of a homogenous space.
As it is shown in \citeBib{Rashevsky} it gives ability to define
concepts of invariance and of geometrical object.

We introduce two types of transformation многообразия базисов:
active and passive transformations. The difference between them is
that the passive transformation can be expressed as a transformation of
an original space.

This definition can be extended on an arbitrary manifold. However in
this case we generalize the definition базиса and introduce a reference
frame. In case of an event space of general relativity it leads us to
a natural definition of a reference frame and the Lorentz transformation.
A reference frame in event space is a smooth field of orthonormal frames.
\fi

Принцип инвариантности, рассмотренный в \citeBib{0412.391},
ограничен векторными пространствами и применим только
в рамках специальной теории относительности. Наша задача
описать конструкции, которые позволяют распространить
принцип инвариантности на общую теорию относительности.

Измерение пространственного интервала и временных отрезков
является одной из важных задач общей теории относительности.
Это физический процесс, который позволяет изучать
геометрию в определённой области пространства времени.
С точки зрения геометрии, наблюдатель пользуется ортогональным базисом в касательной
плоскости как своим измерительным инструментом,
так как ортогональный базис приводит к простейшей локальной геометрии.
Двигаясь от точки к точке, наблюдатель переносит с собой свой измерительный прибор.

Понятие геометрического объекта тесно связано с
физическими величинами, измеряемыми в пространстве времени.
Принцип инвариантности позволяет выразить физические законы
независимо от выбора базиса. С другой стороны, если мы хотим
проверить полученное соотношение в опыте, мы должны зафиксировать
измерительный прибор. В нашем случае - это базис. Выбрав
базис, мы можем определить координаты геометрического
объекта, соответствующего изучаемой физической величине.
Следовательно мы можем определить измеряемое значение.

Каждая система отсчёта снабжена неголономными координатами.
Например, синхронизация системы отсчёта - это неголономная координата времени.
Простые расчёты показывают как синхронизация влияет на измерение времени в
окрестности Земли.
Измерение эффекта Допплера от звезды, вращающейся вокруг чёрной дыры, помогает
определить массу чёрной дыры.

Разделы \ref{section: Time Delay in Central Body Gravitational Field}
и \ref{section: Lorentz Transformation in Orbital Direction}
показывают важность расчётов в ортогональном
базисе. Координаты, которыми мы пользуемся в пространстве событий,
- это просто метки
и расчёты, которые мы выполняем в координатах могут оказаться
не надёжными. Например, в статьях \citeBib{Tartaglia,Tomozawa}
авторы определяют координатную скорость света. Это ведёт к
неверному ответу и в результате этого к
различию скорости света в разных направлениях.

Некоторые авторы используют идею Эйнштейна о переменной скорости света
\citeBib{Ranada}. Тем не менее, Эйнштейн предположил эту идею,
когда собирался создать
теорию тяготения в пространстве Минковского,
и следовательно, он предполагал, что масштаб
пространства и времени не меняются. Когда Эйнштейн познакомился с римановой
геометрией, он изменил своё мнение и никогда
не возвращался к идее о переменной скорости
света. Масштаб пространства и времени и скорость света
являются связанными в современной
теории и мы не можем изменить одну величину без изменения другой.

Некоторые статьи посвящены теории переменной скорости света
\citeBib{Magueijo,Bassett}. Их теория основана на идее, что метрический тензор
может быть инвариантен относительно преобразования подобия. Эта идея не нова.
Как только Эйнштейн опубликовал общую теории относительности,
Вейль предложил свою идею сделать теорию инвариантной относительно
конформного преобразования. Тем не менее, Эйнштейн возражал
этой идее, так как она разрушала зависимость между расстоянием
и собственным временем. Мы можем найти детальный анализ в \citeBib{Straumann}.

Мы имеем тесную связь между скоростью света
и единицами длины и времени в специальной и общей теории относительности.
Когда мы развиваем новую теорию и обнаруживаем, что скорость света меняется,
мы должны спросить себя о причине. Сделали ли мы аккуратное измерение?
Имеем ли мы альтернативный путь для обмена информацией и синхронизации
системы отсчёта? Меняются ли преобразования между системами отсчёта
и образуют ли они группу?

В некоторых моделях фотон может иметь небольшую массу покоя \citeBib{Lammerzahl}.
В этом случае скорость света отлична от максимальной скорости и может
зависеть от направления. Недавний эксперимент \citeBib{Muller}
наложил ограничения на параметры этих моделей.
\fi

\ifx\PrintBook\Defined
\section{Симметрия}

The torsion leads to a change in the Killing equation. We also need to add a similar equation
for the connection.

Ассиметрия связности возникает не только за счёт кручения. Изучение теории
геометрического объекта в векторном пространстве приводит к её естественному
обобщению: теории системы отсчёта в пространстве событий. Система отсчёта
является мощнейшим измерительным инструментом в общей теории относительности.
\fi


==> Refernce.Frame.Russian.tex <==
%auto-ignore
\def\texRefernceFrame{}

\ifx\PrintBook\Defined
				\chapter{Система отсчёта в пространстве событий}
\fi

			\section{Система отсчёта на многообразии}

Мы показали в разделе
\xRef{0412.391}{section: Basis in Vector Space},
что многообразие базисов векторного пространства можно отождествить
с группой симметрий этого пространства.
Нас не интересовали детали строения репера,
и изложенная теория может быть обобщена
и перенесена на произвольное многообразие.
В этом разделе мы  обобщаем определение базиса и определяем систему
отсчёта на многообразии.
В случае пространства событий общей теории относительности это ведёт нас к
естественному определению системы отсчёта и преобразования Лоренца.

Когда мы изучаем многообразие $\mathcal{V}$, геометрия касательного пространства
является одним из важных факторов.
В этом разделе мы предполагаем
\begin{itemize}
\item все касательные пространства имеет одну и ту же геометрию;
\item касательное пространство
является векторным пространством $\mathcal{V}$
конечной размерности $n$;
\item группой симметрии касательного пространства является группа Ли $G$.
\end{itemize}

		\begin{definition}
		\label{definition: type G reference frame}
Mы будем называть множество
\symb{\Basis e=<\Vector e_{(i)},i\in I>}1{reference frame}
векторных полей \symb{\Vector e_{(i)}}1{vector field of reference frame}
\AddIndex{G\Hyph системой отсчёта на многообразии}{G reference frame}
$\mathcal{V}$, если
для любого $x\in\mathcal{V}$ множество
$\Basis e(x)=<\Vector e_{(i)}(x),i\in I>$ является G\Hyph базисом\footnote{Согласно разделу
\xRef{0412.391}{section: Basis in Vector Space}
мы можем
отождествить базис $\Basis e(x)$ с элементом группы $G$.}
в касательном пространстве $T_x$.\footnote{Существование на многообразии $G$\Hyph системы отсчёта
требует доказательства в каждом случае.}
Мы будем пользоваться обозначением
$\ShowSymbol{vector field of reference frame}\in\Basis e$,
для векторных полей, порождающих
$G$\Hyph систему отсчёта $\Basis e$.
		\qed
		\end{definition}

Векторное поле $\Vector a$ имеет разложение	\begin{equation}
\Vector a=a^{(i)}\Vector e_{(i)}
	\label{eq: Vector field expansion, reference frame}
	\end{equation}
относительно системы отсчёта $\Basis e$.

Если мы не ограничим определение системы отсчёта группой симметрии,
мы можем выбрать систему отсчёта
\symb{\Basis\partial=<\Vector \partial_i>}1{coordinate reference frame}
в каждой точке многообразия,
определённую векторными полями, касательными к линиям $x^i=const$.
Это поле базисов мы будем называть \AddIndex{координатной
системой отсчёта}{coordinate reference frame}.
Векторное поле $\Vector a$ имеет разложение
	\begin{equation}
\Vector a=a^i\Vector \partial_i
	\label{eq: Vector field expansion, coordinate reference frame}
	\end{equation}
относительно координатной системы отсчёта.
Тогда стандартные координаты системы отсчёта $\Basis e$ имеют вид
\symb{e^k_{(i)}}1{standard coordinates of reference frame}
	\begin{equation}
\Vector e_{(i)}=e^k_{(i)}\Vector \partial_k
	\label{eq: reference frame expansion relative coordinate reference frame}
	\end{equation}
Так как векторы $\Vector e_{(i)}$ линейно независимы в каждой точке, матрица
$\|e^k_{(i)}\|$ имеет обратную матрицу $\|e_k^{(i)}\|$
	\begin{equation}
\Vector \partial_k=e_k^{(i)}\Vector e_{(i)}
	\label{eq: coordinate reference frame expansion relative reference frame}
	\end{equation}

Мы
также пользуемся более широким определением для
системы отсчёта на многообразии,
представленное в виде
\symb{\Basis e=(\Vector e_{(k)},\Vector e^{(k)})}1
{reference frame, extensive definition},
где мы задаём множество векторное полей
$\Vector e_{(k)}$ и двойственных им форм
\symb{\Vector e^{(k)}}1{dual forms, reference frame}
таких, что
	\begin{equation}
\Vector e^{(k)}(\Vector e_{(l)})=\delta^{(k)}_{(l)}
	\label{eq: dual forms and vector fields}
	\end{equation}
в каждой точке.
Формы $\Vector e^{(k)}$ определены однозначно из
\eqref{eq: dual forms and vector fields}.

Подобным образом мы можем определить
координатную систему отсчёта
\symb{(\Vector \partial_i,\Vector ds^i)}1
{coordinate reference frame, extensive definition}.
Эти системы отсчёта связаны отношением
	\begin{align}
	\label{eq: holonomic and anholonomic vector field}
\Vector e_{(k)}&=e_{(k)}^i\Vector \partial_i\\
	\label{eq: holonomic and anholonomic forms}
\Vector e^{(k)}&=e^{(k)}_i\Vector dx^i
	\end{align}
Из равенств
\eqref{eq: holonomic and anholonomic vector field},
\eqref{eq: holonomic and anholonomic forms},
\eqref{eq: dual forms and vector fields} следует
	\begin{equation}
e^{(k)}_ie^i_{(l)}=\delta^{(k)}_{(l)}
	\label{eq: frame and coframe}
	\end{equation}

В частности, мы предположим, что мы имеем $GL(n)$-систему отсчёта 
$(\partial,dx)$, порождённый $n$ дифференцируемыми векторными полями
$\partial_i$ и 1-формами $dx^i$, которые определяют поля базисов $\partial$
и кобазисов $dx$, дуальных им.

Если задана функция $\varphi$ on $V$, то мы определяем \AddIndex{пфаффову производную}{pfaffian derivative}
\[d\varphi=\partial_i\varphi dx^i\]

\section{Система отсчёта в пространстве событий}

Начиная с этого раздела, мы будем рассматривать ортогональную систему отсчёта
$\Basis e=(\Vector e_{(k)},\Vector e^{(k)})$
в римановом пространстве с метрическим тензором $g_{ij}$.
Согласно определению, в каждой точке риманова пространства
векторные поля ортогональной системы отсчёта удовлетворяют соотношению
\[
g_{ij}e^i_{(k)}e^j_{(l)}=g_{(k)(l)}
\]
где $g_{(k)(l)}=0$, если $(k)\ne(l)$, и $g_{(k)(k)}=1$
или $g_{(k)(k)}=-1$ в зависимости от сигнатуры метрики.

Мы можем определить
\AddIndex{систему отсчёта в пространстве событий}
{reference frame in event space}
$V$ как $O(3,1)$\Hyph систему отсчёта.
Для нумерации векторов мы пользуемся индексом
$k=0, ..., 3$. Индекс $k=0$ соответствует времени подобному векторному полю.

		\begin{remark}
		\label{remark: existence of a reference frame}
Мы можем доказать существование системы отсчёта, пользуясь
процедурой ортогонолизации в каждой точке пространства
времени. Из той же процедуры мы видим, что координаты базиса
непрерывно зависят от точки.

Непрерывное поле времениподобных векторов каждого базиса определяет
конгруэнцию линий, касательных этому полю.
Мы будем говорить, что каждая из этих линий является мировой линией
наблюдателя или \AddIndex{локальной системой отсчёта}{local reference frame}.
Следовательно, система отсчёта - это множество локальных систем отсчёта.
		\qed
		\end{remark}

Мы определяем \AddIndex{преобразование Лоренца}{Lorentz transformation}
как преобразование системы отсчёта
$$
{x'}^i = f^i (x^0, x^1, x^2, x^3)
$$
\begin{equation}
{e'}^i_{(k)} = a^i_j b^{(l)}_{(k)} e^j_{(l)}
\label{LorentzTransformation}
\end{equation}
где
$$
a^i_j = \frac {\partial x'^i} {\partial x'^j}
$$
$$
\delta_{(i)(l)} b^{(i)}_{(j)} b^{(l)}_{(k)} = \delta_{(j)(k)}
$$
Мы будем называть преобразование $a^i_j$ голономной частью и преобразование $b^{(l)}_{(k)}$
неголономной частью.

\section{Неголономные координаты}

Пусть $E(V, G,\pi)$ - главное расслоение,
где $V$ - дифференцируемое многообразие размерности $n$ и класса
не меньше, чем $2$. Мы также положим, что $G$ - группа симметрии касательной плоскости.

Мы определим форму связности на главном расслоении 
	\begin{equation}
\omega^L=\lambda^L_Nda^N+\Gamma^L_idx^i\ \ \ \omega=\lambda_Nda^N+\Gamma dx
	\label{eq: G connection form}
	\end{equation}
Мы называем функции $\Gamma_i$ компонентами связности.

Если слой является группой $GL(n)$, то связность имеет вид
	\begin{equation}
\omega^a_b=\Gamma^a_{bc}dx^c
	\label{eq: GLn connection form}
	\end{equation}
\[\Gamma^A_i=\Gamma^a_{bi}\]

Векторное поле $\Vector a$ имеет два вида координат: \AddIndex{голономные координаты}{vector holonomic coordinates}
\symb{a^i}1{vector holonomic coordinates} относительно координатной системы отсчёта
и \AddIndex{неголономные координаты}{vector anholonomic coordinates}
\symb{a^{(i)}}1{vector anholonomic coordinates}
относительно системы отсчёта. Эти два вида координат так же следуют отношению
	\begin{equation}
a^i(x)=e^i_{(i)}(x)a^{(i)}(x)
	\label{eq: parallel transfer, 3}
	\end{equation}
в любой точке $x$.

Мы можем изучать параллельный перенос векторных полей, пользуясь любой формой координат.
Так как \eqref{LorentzTransformation} - линейное преобразование,
мы ожидаем, что параллельный перенос в
неголономных координатах имеет такое же представление, как в голономных координатах.
Таким образом мы запишем
\[
da^k=-\Gamma^k_{ij}a^idx^j
\]
\[
da^{(k)}=-\Gamma^{(k)}_{(i)(j)}a^{(i)}dx^{(j)}
\]
Необходимо установить связь между
\AddIndex{голономными координатами связности}{holonomic coordinates of connection}
\symb{\Gamma^k_{ij}}1{holonomic coordinates of connection}
и \AddIndex{неголономными координатами связности}{anholonomic coordinates of connection}
\symb{\Gamma^{(k)}_{(i)(j)}}1{anholonomic coordinates of connection}
	\begin{equation}
a^i(x+dx)=a^i(x)+da^i=a^i(x)-\Gamma^i_{kp}a^k(x)dx^p
	\label{eq: parallel transfer, 1}
	\end{equation}
	\begin{equation}
a^{(i)}(x+dx)=a^{(i)}(x)+da^{(i)}=a^{(i)}(x)-\Gamma^{(i)}_{(k)(p)}a^{(k)}(x)dx^{(p)}
	\label{eq: parallel transfer, 2}
	\end{equation}
Предполагая \eqref{eq: parallel transfer, 1},
\eqref{eq: parallel transfer, 2} и \eqref{eq: parallel transfer, 3}, мы получим
	\begin{equation}
\begin{matrix}
a^i(x)-\Gamma^i_{kp}a^k(x)dx^p\\
=e^i_{(i)}(x+dx)
\left(a^{(i)}(x)-\Gamma^{(i)}_{(k)(p)}e^{(k)}_i(x)a^i(x)e^{(p)}_p(x)dx^p\right)
\end{matrix}
	\label{eq: parallel transfer, 4}
	\end{equation}
Из \eqref{eq: parallel transfer, 4} следует, что 
	\begin{align*}
\Gamma^{(i)}_{(k)(p)}e^{(k)}_i(x)e^{(p)}_p(x)a^i(x)dx^p
&=a^{(i)}(x)-e^{(i)}_i(x+dx)\left(a^i(x)-\Gamma^i_{kp}a^k(x)dx^p\right)\\
&=a^i(x)e^{(i)}_i(x)-e^{(i)}_i(x+dx)\left(a^i(x)-\Gamma^i_{kp}a^k(x)dx^p\right)\\
&=a^i(x)\left(e^{(i)}_i(x)-e^{(i)}_i(x+dx)\right)
+e^{(i)}_j(x)\Gamma^j_{ip}a^i(x)dx^p\\
&=e^{(i)}_j(x)\Gamma^j_{ip}a^i(x)dx^p
-a^i(x)\frac{\partial e^{(i)}_i(x)}{\partial x^p}dx^p\\
&=\left(e^{(i)}_j(x)\Gamma^j_{ip}
-\frac{\partial e^{(i)}_i(x)}{\partial x^p}\right)a^i(x)dx^p
	\end{align*}
Так как $a^i(x)$ и $dx^p$ произвольны, мы имеем 
	\[
\Gamma^{(i)}_{(k)(p)}e^{(k)}_i(x)e^{(p)}_p(x)
=e^{(i)}_j(x)\Gamma^j_{ip}
-\frac{\partial e^{(i)}_i(x)}{\partial x^p}
	\]
	\begin{equation}
\Gamma^{(i)}_{(k)(p)}
=e^i_{(k)}e^p_{(p)}e^{(i)}_j\Gamma^j_{ip}
-e^i_{(k)}e^p_{(p)}\frac{\partial e^{(i)}_i}{\partial x^p}
	\label{eq: parallel transfer, 5}
	\end{equation}
Мы определим символический оператор
	\begin{equation}
\frac{\partial}{\partial x^{(p)}}
=e^p_{(p)}\frac{\partial}{\partial x^p}
	\label{eq: anholonomic derivative}
	\end{equation}
Из \eqref{eq: frame and coframe} следует
	\begin{equation}
e^i_{(l)}\frac{\partial e^{(k)}_i}{\partial x^p}+
e^{(k)}_i\frac{\partial e^i_{(l)}}{\partial x^p}=0
	\label{eq: parallel transfer, 6}
	\end{equation}
Подставим \eqref{eq: anholonomic derivative} и
\eqref{eq: parallel transfer, 6} в \eqref{eq: parallel transfer, 5}
\begin{equation}
\Gamma^{(i)}_{(k)(p)}=
e^i_{(k)}e^p_{(p)}e^{(i)}_j\Gamma^j_{ip}
-e^{(i)}_i\frac{\partial e^i_{(k)}}{\partial x^{(p)}}
\label{eq: Gamma1}
\end{equation}

Равенство \eqref{eq: Gamma1} показывает некоторое сходство между голономными и неголономными координатами.
Мы определим символ \symb{\partial_{(k)}}1{partial(k)} для производной вдоль векторных полей $e_{(k)}$
$$\partial_{(k)}=e^i_{(k)}\partial_i$$
Тогда \eqref{eq: Gamma1} принимает форму
$$
\Gamma^{(k)}_{(l)(p)}=
e^i_{(l)}e^r_{(p)}e^{(k)}_j\Gamma^j_{ir}
-e^i_{(l)}\partial_{(p)} e^{(k)}_i
$$

Следовательно, когда мы переходим от голономных координат к неголономным, преобразование связности
подобно преобразованию при переходе от одной координатной системы к другой.
Это приводит нас к модели неголономных координат.

Векторные поля $e_{(k)}$ порождают кривые, определённые дифференциальными уравнениями
$$
e^j_{(l)} \frac{\partial t} {\partial x^j} = \delta^{(k)}_{(l)}
$$
или символической системой 
\begin{equation}
\frac{\partial t} {\partial x^{(l)}} = \delta^{(k)}_{(l)}
\label{DefForX}
\end{equation}
Имея в виду символическую систему \eqref{DefForX}, мы обозначим
функционал $t$ посредством \symb{x^{(k)}}1{x(k)}
и будем называть его
\AddIndex{неголономной координатой}{anholonomic coordinate}.
Мы будем называть обычные координаты голономными.

Отсюда мы можем найти производную и получить
\begin{equation}
\frac{\partial x^{(i)}} {\partial x^k} = e^{(i)}_k
\label{DerivativeForX}
\end{equation}
Необходимое и достаточное условие полной интегрируемости
системы \eqref{DerivativeForX} - это равенство
$$
c^{(i)}_{(k)(l)} =0
$$
где мы вводим \AddIndex{объект неголономности}{anholonomity object}
\symb{c^{(i)}_{(k)(l)}}0{anholonomity object}
	\begin{equation}
\ShowSymbol{anholonomity object} =e^k_{(k)}e^l_{(l)}
\left(
\frac{\partial e^{(i)}_k}{\partial x^l} - \frac{\partial e^{(i)}_l}{\partial x^k}
\right)
	\label{eq: Anholonomity Object}
	\end{equation}
Следовательно, любая система отсчёта имеет $n$ векторных полей
$$
\partial_{(k)} = \frac\partial {\partial x^{(k)}} = e^i_{(k)} \partial_i
$$
которые имеют коммутатор
$$
[\partial_{(i)},\partial_{(j)}]=
\left( e^k_{(i)}\partial_k e^l_{(j)} - e^k_{(j)}\partial_k e^l_{(i)}\right)e^{(m)}_l \partial_{(m)}=$$
$$e^k_{(i)}e^l_{(i)}\left( -\partial_k e_l^{(m)} + \partial_l e_l^{(m)}\right)\partial_{(m)}=
c^{(m)}_{(k)(l)}\partial_{(m)}
$$
По той же причине мы определяем форму
$$dx^{(k)}=e^{(k)}=e^{(k)}_l dx^l$$
и внешний дифференциал этой формы имеет вид
	\begin{equation}
	\begin{split}
d^2x^{(k)}&=d\left( e^{(k)}_i dx^i\right)\\
&=\left(\partial_j e_i^{(k)} -\partial_i e_j^{(k)}\right)dx^i \wedge dx^j\\
&=-c^{(m)}_{(k)(l)}dx^{(k)}\wedge dx^{(l)}
	\end{split}
	\label{eq: anholonomity}
	\end{equation}

Следовательно, когда $c^{(i)}_{(k)(l)} \not =0$, дифференциал $dx^{(k)}$ не является точным дифференциалом
и система \eqref{DerivativeForX} вообще говоря не может быть интегрируемой.
Тем не менее, мы можем построить реальный объект, который
моделирует решение. Мы можем изучать, как функция $x^{(i)}$ изменяется
вдоль разных кривых.
Мы будем называть такие координаты \AddIndex{неголономными координатами на многообразии}
{anholonomic coordinates on manifold}.

		\begin{remark}
		\label{remark: anholonomic coordinates, model}
Функция $x^{(i)}$ является натуральным параметром вдоль кривой потока
векторных полей $\Vector e_{(i)}$.
Пример такой функции мы рассмотрим в разделе
\ref{section: Synchronization of Reference Frame}.
Cобственное время определено вдоль мировой линии локальной системы
отсчёта. Как мы видели в замечании
\ref{remark: existence of a reference frame}
всё пространство пронизано мировыми линиями локальных систем.
Чтобы собственное время локальных систем могло быть
временем системы отсчёта,
мы ожидаем, что собственное время непрерывно изменяется
от точки к точке. Для синхронизации часов локальных систем отсчёта
мы пользуемся классической процедурой обмена световыми сигналами.

С точки зрения математики
– это проблема интегрирования дифференциальной формы.
Тем не менее, изменение функции вдоль петли имеет вид
	\begin{equation}
	\begin{split}
\Delta x^{(i)}
&= \oint dx^{(i)}\\
&=\int\int c^{(i)}_{(k)(l)}dx^{(k)}\wedge dx^{(l)}\\
&=\int\int c^{(i)}_{(k)(l)} e^{(k)}_k e^{(l)}_l dx^k\wedge dx^l
	\end{split}
	\label{eq: change of coordinate along a loop}
	\end{equation}

На первый взгляд возникает ощущение, что нельзя синхронизировать часы,
чего мы не наблюдаем на практике.
Мы допускаем, что синхронизация возможна до тех пор,
пока мы определяем время вдоль незамкнутых кривых.
Синхронизация нарушается, когда мы пытаемся синхронизировать часы
вдоль замкнутой кривой.

Это означает неоднозначность определения неголономной координаты.
		\qed
		\end{remark}

Начиная с этого места, мы не будем делать различия между голономными и неголономными координатами.
Мы так же будем обозначать $b^{(l)}_{(k)}$ как ${a^{-1}}^{(l)}_{(k)}$ в преобразовании Лоренца
\eqref{LorentzTransformation}.

Хотя форма $dx^{(k)}$ не является точным дифференциалом, нетрудно убедиться,
что форма $d^2x^{(k)}$ является внешним дифференциалом формы $dx^{(k)}$.
Следовательно,
	\begin{equation}
	\label{eq: exterior derivative 3}
d^3x^{(k)}=0
	\end{equation}

Мы можем представить внешний дифференциал формы, записанной в неголономных
координатах, в виде
\begin{align*}
&d(a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge dx^{(i_n)})\\
=&a_{(i_1)...(i_n),p}dx^p\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}\\
-&a_{(i_1)...(i_n)}ddx^{(i_1)}\wedge ...\wedge dx^{(i_n)}-...
-(-1)^{n-1}a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge ddx^{(i_n)}\\
=&a_{(i_1)...(i_n),(p)}e_p^{(p)}e^p_{(r)}dx^{(r)}\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}\\
-&a_{(i_1)...(i_n)}c^{(i_1)}_{(p)(r)}dx^{(p)}\wedge dx^{(r)}\wedge ...\wedge dx^{(i_n)}-...\\
-&(-1)^{n-1}a_{(i_1)...(i_n)}dx^{(i_1)}\wedge ...\wedge c^{(i_n)}_{(p)(r)}dx^{(p)}\wedge dx^{(r)}\\
=&(a_{(i_1)...(i_n),(p)}
-a_{(r)...(i_n)}c^{(r)}_{(p)(i_1)}-...
-a_{(i_1)...(r)} c^{(r)}_{(p)(i_n)})
dx^{(p)}\wedge dx^{(i_1)}\wedge ...\wedge dx^{(i_n)}
\end{align*}
В случае формы $d^3x^{(k)}$ мы получим равенство
\begin{equation}
	\label{eq: exterior derivative, anholonomic form}
\begin{array}{l}
d(c^{(k)}_{(i)(j)}dx^{(i)}\wedge dx^{(j)})\\
=(c^{(k)}_{(i)(j),(p)}
-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}  
\end{array}
\end{equation}
Из равенств \eqref{eq: exterior derivative 3}
и \eqref{eq: exterior derivative, anholonomic form}
следует
\begin{equation}
	\label{eq: exterior derivative, anholonomic form, 1}
(c^{(k)}_{(i)(j),(p)}
-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}=0  
\end{equation}
Нетрудно убедиться, что
\begin{equation}
	\label{eq: exterior derivative, anholonomic form, 2}
\begin{array}{l}
(-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
-c^{(k)}_{(i)(r)} c^{(r)}_{(p)(j)})
dx^{(i)}\wedge dx^{(j)}\\
=(-c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
+c^{(k)}_{(r)(i)} c^{(r)}_{(p)(j)})
dx^{(i)}\wedge dx^{(j)}\\
=-2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
dx^{(i)}\wedge dx^{(j)}
\end{array}
\end{equation}
Подставив \eqref{eq: exterior derivative, anholonomic form, 2}
в \eqref{eq: exterior derivative, anholonomic form, 1}, получим
\begin{equation}
	\label{eq: exterior derivative, anholonomic form, 3}
(c^{(k)}_{(i)(j),(p)}
-2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)})
dx^{(p)}\wedge dx^{(i)}\wedge dx^{(j)}=  0
\end{equation}
Из \eqref{eq: exterior derivative, anholonomic form, 3} следует
\begin{equation}
	\label{eq: exterior derivative, anholonomic form, 4}
\begin{array}{l}
c^{(k)}_{(i)(j),(p)}+c^{(k)}_{(j)(p),(i)}+c^{(k)}_{(p)(i),(j)}\\
=2c^{(k)}_{(r)(j)}c^{(r)}_{(p)(i)}
+2c^{(k)}_{(r)(p)}c^{(r)}_{(i)(j)}
+2c^{(k)}_{(r)(i)}c^{(r)}_{(j)(p)}
\end{array}
\end{equation}

Мы определим форму кривизны для связности \eqref{eq: G connection form}
\[\Omega=d\omega+[\omega,\omega]\]
\[\Omega^D=d\omega^D+C^D_{AB}\omega^A\wedge \omega^B=R^D_{ij}dx^i\wedge dx^j\]
где мы определяем объект кривизны
\[R^D_{ij}=\partial_i\Gamma^D_j-\partial_j\Gamma^D_i+C^D_{AB}\Gamma^A_i\Gamma^B_j+\Gamma^D_k c^k_{ij}\]

Форма кривизны для связности \eqref{eq: GLn connection form} is
	\begin{equation}
\Omega^a_c = d \omega^a_c + \omega^a_b \wedge \omega^b_c
	\label{eq: Curvature}
	\end{equation}
где мы определим объект кривизны
	\begin{equation}
R^D_{ij}=R^a_{bij}=\partial_i\Gamma^a_{bj}-\partial_j\Gamma^a_{bi}
+\Gamma^a_{ci}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{bi}+\Gamma^a_{bk} c^k_{ij}
	\label{eq: GLn curvature}
	\end{equation}
Мы определим тензор Ричи
\[R_{bj}=R^a_{baj}=\partial_a\Gamma^a_{bj}-\partial_j\Gamma^a_{ba}
+\Gamma^a_{ca}\Gamma^c_{bj}-\Gamma^a_{cj}\Gamma^c_{ba}+\Gamma^a_{bk} c^k_{aj}\]

\ifx\texFuture\Defined
			\section{Covariant exterior Derivative}

exterior derivative of form \eqref{eq: holonomic and anholonomic forms}
is different from 0. At first sight it looks unusual. However
form \eqref{eq: holonomic and anholonomic forms} is not
exact differential.

мы define covariant exterior derivative of form $t = t_a \theta^a$ as
\[
Dt = t_{a;b} \theta^b \land \theta^a
+ t_a c^a_{bc} \theta^b \land \theta^c
\]

When мы look at such equation мы ask if $d^2=0$ still is legal.

			\section{Moving Basis}

мы meet another interesting situation when мы study moving of frame along
manifold. If мы introduce derivative for each vector of frame as
$$
\frac {De^i_{(k)}} {dx^l}
= e^i_{(k),l} + \Gamma^i_{pl} e^p_{(k)}
$$
then мы get transformation for moving frame
$$
\frac {De^i_{(k)}} {dx^l}
= A^{(p)}_{(k)l} e^i_{(p)}
$$
\[
A_{(p)(k)l} + A_{(k)(p)l} = - g_{(p)(k);l}
\]
In particular,
\[A_{(k)(k)l}= - \frac 1 2 g_{(k)(k);l}\]
мы observed the same type of transformation when мы analyzed Frenet transfer.

Therefore, if $g_{pk;l} = 0$, then мы get orthogonal transformation of frame.
However this is not so in case of nonzero derivative.
\fi


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb{texBiring}%
   {$(^{\gi a}_{\gi b})$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb{texBiring}%
   {минор}%
   {A from b a}%
\Symb{texBiring}%
   {минор}%
   {A from columns T}%
\Symb{texBiring}%
   {минор}%
   {A from rows S}%
\Symb{texBiring}%
   {минор}%
   {A without column a}%
\Symb{texBiring}%
   {минор}%
   {A without columns T}%
\Symb{texBiring}%
   {минор}%
   {A without row b}%
\Symb{texBiring}%
   {минор}%
   {A without rows S}%
\Symb{texPolymodule}%
   {активное преобразование}%
   {active transformation}%
\Symb{texTypeBasis}%
   {аффинное пространство}%
   {affine space}%
\Symb{texBasis}%
   {аффинное пространство}%
   {An}%
\Symb{texBiring}%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb{texBiring}%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb{texBiring}%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb{texBiring}%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb{texVectorSpace}%
   {\dcr вектор}%
   {dcr vector}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb{texLie}%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb{texLie}%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb{texVectorSpace}%
   {\drc вектор}%
   {drc vector}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb{texPolymodule}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texBiring}%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb{texBiring}%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb{texBiring}%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb{texBiring}%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb{texBiring}%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb{texTstarRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texFiberedGroup}%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb{texTstarRepresentation}%
   {левый сдвиг}%
   {Tstar shift}%
\Symb{texFiberedGroup}%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb{texRefernceFrame}%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb{texRefernceFrame}%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%
\Symb{texBasis}%
   {многообразие базисов аффинного пространства}%
   {BAn}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства $\mathcal{V}$}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb{texBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb{texBasis}%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb{texBundle}%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Symb{texBundle}%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb{texTypeBasis}%
   {многообразие базисов аффинного пространства}%
   {FAn}%
\Symb{texTypeBasis}%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb{texTypeBasis}%
   {многообразие базисов евклидова пространства}%
   {FEn}%

\SetIndexSpace%
\Symb{texBasis}%
   {центро-аффинное пространство}%
   {CAn}%
\Symb{texTypeBasis}%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb{texLie}%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb{texLie}%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb{texLieRepresentation}%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to drc vector space}%
\Symb{texCalculus}%
   {дифференциал функции}%
   {differential, drc vector space to skew field}%
\Symb{texVectorSpace}%
   {\drc координатное векторное пространство}%
   {drc coordinate vector space}%
\Symb{texVectorSpace}%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace D}%
\Symb{texAffine}%
   {производная}%
   {overline D}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 1, skew field}%
\Symb{texVectorSpace}%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb{texTidal}%
   {скорость отклонения}%
   {speed of deviation}%
\Symb{texVectorSpace}%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%
\Symb{texTypeBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texBasis}%
   {аффинный базис}%
   {Affine Basis}%
\Symb{texTypeBasis}%
   {базис}%
   {basis}%
\Symb{texBasis}%
   {базис векторного пространства}%
   {Basis e}%
\Symb{texBasis}%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb{texVectorSpace}%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb{texPolymodule}%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb{texCartesian}%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb{texBasis}%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb{texRefernceFrame}%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb{texBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {евклидово пространство}%
   {En}%
\Symb{texTypeBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texBasis}%
   {псевдоевклидово пространство}%
   {Enm}%
\Symb{texFiberedAlgebra}%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb{texBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb{texBasis}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texRefernceFrame}%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb{texRefernceFrame}%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb{texBasis}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb{texVectorSpace}%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb{texVectorSpace}%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb{texDiffEq}%
   {центро-аффинный}%
   {Central Affine Basis}%
\Symb{texBundle}%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb{texBundleRelation}%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb{texFiberedAlgebra}%
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb{texCartesian}%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb{texTstarRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%
\Symb{texTypeBasis}%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb{texRefernceFrame}%
   {система отсчёта}%
   {reference frame}%
\Symb{texRefernceFrame}%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb{texPolymodule}%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb{texPolymodule}%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%
\Symb{texVectorSpace}%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb{texFiberedMorphism}%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb{texFiberedMorphism}%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb{texLie}%
   {алгебра Ли группы Ли}%
   {g}%
\Symb{texLie}%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb{texTypeBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texBasis}%
   {группа аффинных преобразований}%
   {GLAn}%
\Symb{texLie}%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb{texBasis}%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb{texTstarRepresentation}%
   {малая группа элемента $x$}%
   {little group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective starT covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective starT covariant representation of group}%
\Symb{texFiberedGroup}%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective Tstar covariant representation of fibered group}%
\Symb{texTstarRepresentation}%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective Tstar covariant representation of group}%
\Symb{texVectorSpace}%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb{texTstarRepresentation}%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%
\Symb{texBiring}%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb{texLinearMap}%
   {\rcd векторное пространство \drc линейных отображений}%
   {rcd vector space of drc linear maps}%

\SetIndexSpace%
\Symb{texLieRepresentation}%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb{texLinearLie}%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%
\Symb{texRepresentation}%
   {левый сдвиг}%
   {left shift}%
\Symb{texDiffProperty}%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb{texDiffProperty}%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb{texBundleRelation}%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb{texBasis}%
   {пассивное преобразование}%
   {passive transformation}%
\Symb{texRepresentation}%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texTstarMorphism}%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb{texTstarMorphism}%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb{texTstarRepresentation}%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb{texTstarRepresentation}%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%
\Symb{texBasis}%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb{texBasis}%
   {геометрический объект}%
   {geometrical object, vector space}%
\Symb{texFiberedGroup}%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb{texRepresentation}%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоение}%
   {bundle}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb{texFiberedMorphism}%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb{texCartesian}%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb{texFiberedAlgebra}%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%
\Symb{texBasis}%
   {активное преобразование}%
   {active transformation}%
\Symb{texAffine}%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb{texVectorSpace}%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb{texAffine}%
   {кривизна}%
   {GLn curvature_overline}%
\Symb{texVectorSpace}%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb{texRepresentation}%
   {правый сдвиг}%
   {right shift}%
\Symb{texRepresentation}%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb{texBundleRelation}%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb{texBundleRelation}%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb{texVectorSpace}%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%
\Symb{texLie}%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%
\Symb{texBasis}%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb{texBasis}%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb{texVectorSpace}%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb{texVectorSpace}%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb{texLinearMap}%
   {($S$, $T$)\hyph бимодуль}%
   {R S bimodule}%
\Symb{texVectorSpace}%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb{texVectorSpace}%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb{texBasis}%
   {векторное пространство}%
   {V}%

\SetIndexSpace%
\Symb{texPolymodule}%
   {геометрический объект в координатном представлении,		определённом в векторном пространстве}%
   {geometrical object, coordinate vector space}%
\Symb{texPolymodule}%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%

\SetIndexSpace%
\Symb{texTidal}%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb{texRepresentation}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texTstarMorphism}%
   {тождественное преобразование}%
   {identical transformation}%
\Symb{texBasis}%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb{texBiring}%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb{texAffine}%
   {символ Картана}%
   {Cartan symbol}%
\Symb{texAffine}%
   {связность}%
   {conection overline}%
\Symb{texRefernceFrame}%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb{texAffine}%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb{texBundle}%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%
\Symb{texLie}%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb{texLie}%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb{texLie}%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%
\Symb{texRefernceFrame}%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb{texCalculus}%
   {частная производная отображения $\Vector f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, drc vector space}%
\Symb{texCalculus}%
   {частная производная отображения $f$ по переменной $v^{\gi a}$}%
   {partial derivative of mapping, 2, skew field}%
\Symb{texRefernceFrame}%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%

\SetIndexSpace%
\Symb{texLie}%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb{texAffine}%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%
\Symb{texBundleRelation}%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%
\Symb{texCartesian}%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb{texCartesian}%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%
\Symb{texBundle}%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb{texBundle}%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

